On the Impossibility of Convergence of Mixed Strategies with No Regret Learning

We study the limiting behavior of the mixed strategies that result from optimal no-regret learning strategies in a repeated game setting where the stage game is any 2 by 2 competitive game. We consider optimal no-regret algorithms that are mean-based and monotonic in their argument. We show that for any such algorithm, the limiting mixed strategies of the players cannot converge almost surely to any Nash equilibrium. This negative result is also shown to hold under a broad relaxation of these assumptions, including popular variants of Online-Mirror-Descent with optimism and/or adaptive step-sizes. Finally, we conjecture that the monotonicity assumption can be removed, and provide partial evidence for this conjecture. Our results identify the inherent stochasticity in players' realizations as a critical factor underlying this divergence in outcomes between using the opponent's mixtures and realizations to make updates.

==> tex/intro_long.tex <==
%!TEX root = ../main.tex

\section{Introduction}

% {\color{red} Vidya: as I write this I feel like a lot of the ``related work" could just be folded in here.}

The mixed-strategy Nash equilibrium (NE) of a multi-player game is the oldest solution concept in one-shot game theory.
Its existence for all games having a finite pure strategy space was one of the first central results in game theory \citep{von1945theory,nash1951non}, but a finer understanding of how the NE arises as an outcome of repeated, ``natural" play remains a somewhat elusive goal as well as an active area of research\footnote{It is interesting to note that a question that is somewhat pre-requisite to this goal is that of whether the equilibrium can even be computed efficiently --- and even this has been shown to be impossible for general-sum games in the algorithmic game theory community(~\cite{daskalakis2009complexity}). However, for special classes of games, such as zero (or constant-sum) games, it is well-known that the computation of the NE reduces to the computation of a special linear program (LP).}.
Of special interest is whether players who use certain \textit{learning dynamics}, based on principles of minimizing regret with respect to the best response to the empirical average of the opponent's plays\footnote{The first choice of dynamics satisfying this property was introduced in 1957(~\cite{hannan1957approximation}); this was refined a few decades later in a number of algorithms in the \textit{online learning} literature in the 1990s(~\cite{littlestone1989weighted,freund1999adaptive,kalai2005efficient}).
}, are able to converge to equilibrium.
{\color{red} Vidya: Earlier, I had phrased this as connecting no-regret to some notion of \textit{optimality} in repeated zero-sum games: I'm not actually sure that is true if you read Hannan/Blackwell's older papers. 
The only claims made in these papers are in optimality of min-max regret, not min-max loss.
I feel like in general the concept of ``regret" has not seen sufficient scrutiny, and it was invented because very nice guarantees could be obtained on it; not necessarily because it's natural.
}
\mycomment{Maybe we can bring in the motivation for no-regret from the learning in CS literature. Over there it seems to be an established concept commonly used in multi-armed bandits type scenarios. Although you are right, we need an explanation why a player would insist on playing an optimal no-regret strategy. I think a good strategy would be to give several examples of use of no-regret and say it upfront that we would like our players to have optimal no-regret. Better to keep it short and straight-forward to avoid the typical criticisms of no-regret learning in general. For example, structure the argument like if the reader is ready to accept that a player should play optimal no-regret then we have some interesting results, and several other researchers have looked at some version of this, give examples.}
Being learning dynamics, they are fundamentally \textit{uncoupled}, in the sense that the players only use knowledge of their own payoff function, and not their opponents', to update their strategies.
Classical research in the economics(~\cite{foster1997calibrated,foster1998asymptotic,hart2000simple,hart2005adaptive}) as well as computer science(~\cite{freund1999adaptive,blum2007external}) communities has shown that when players play commonly used``no-regret" algorithms against each other, the \textit{time-average} of their strategies will converge (almost surely) to Nash equilibrium when the game being played is zero-sum, or constant-sum\footnote{Convergence to NE does not occur for general non-zero-sum games; in fact, classes of non-zero-sum games have been constructed for which no choice of uncoupled dynamics can lead to even time-averaged convergence to NE(~\cite{hart2003uncoupled}). However, algorithms that satisfy a further refined notion of \textit{internal} no-regret can be shown to converge to the polytope of correlated equilibria of any general game (for a general discussion, see(~\cite[Chapter 4]{nisan2007algorithmic})).}.
{\color{red} Vidya: there is some subtle mis-attribution here: most of the econ references are actually for calibrated learning, which is related to no-internal-regret dynamics, and directly show convergence to the set of correlated equilibria.}

A subtle point here is that the above guarantee --- on convergence of the \textit{time averages} to NE --- does not necessarily imply that the day-to-day behavior converges.
That is, the actual mixed strategy used by each player need not converge to the NE.
Stated alternatively, the \textit{last-iterate} of the player's strategies can diverge.
Consider the \textit{matching pennies} (more common variants of this with $> 2$ strategies are the rock-paper-scissors game) game, in which the pure strategy space for both players is $\{H,T\}$ and the unique mixed-strategy NE for the game consists of the uniform distribution over $\{H,T\}$ for both players.
Clearly, the time average of the dynamic where the players repeatedly cycle through the pure strategies $\{(H,H),(H,T),(T,H),(T,T)\}$ converges to NE --- but the last-iterate by definition cycles, therefore diverges.
In fact, a surprising property was discovered for multiplicative weights/Mirror Descent families of algorithms recently on games like matching pennies(~\cite{bailey2018multiplicative}): while the time average of the players' strategies converges, the individual strategies, or the last-iterate, converges to a limit cycle.
\mycomment{I like this paragraph. Can we start the paper with this, with suitable modifications?}

The question naturally arise whether last-iterate divergence is a specific property of multiplicative weights/Mirror Descent-style algorithms, or a fundamental consequence of the property of no-regret itself.
This paper provides substantial evidence that it is the latter, by proving lack of last-iterate convergence for a broad class of generic no-regret algorithms under minimal assumptions.
{\color{red} Vidya: ``minimal assumptions" is intentionally vague at this stage; I intend to flesh out later.}
Moreover, the setting considered actually corresponds to the actual repeated game setting in which players can only observe the opponent's realizations of their mixed strategies (as opposed to the strategy itself, which is assumed in some recent literature(~\cite{bailey2018multiplicative,daskalakis2018last})).
The ensuing stochasticity in realizations is shown to be one of the critical ingredients (in addition to others) underlying last-iterate divergence.
\mycomment{I like the motivation. My suggestion is we should try to compress these three paragraphs, maybe into one (or two) short paragraph, and begin the paper and later go into more detailed descriptions of these in related work maybe. This way it will be clear at the onset what our paper's goal is. Currently it seems masked and leads one to believe that we are proving some very general result about Nash equilibrium through learning in games. Also many times people are aware of the background, especially in the learning community, and they want to cut to chase.}

\subsection{Our contributions}

We consider the ensemble of $2 \times 2$ \textit{zero-sum games} for which at least one NE is strictly mixed for both players.
Moreover, the game is assumed to have no strictly dominant strategies for either player.
Then, we show the following result (for a formal statement, see Theorem~\ref{thm:lastiterateconvergence}).

\textit{Even if one of the players has already converged to their NE strategy, the other player necessarily diverges in their last iterate, if she is constrained to use a strategy that is no-regret AND a functional of the empirical averages of the other player's realized plays.}

{\color{red} Vidya: as I think about it more, our theorem statement should also hold for functionals of empirical averages of \textit{bounded} functions of the other player's realized plays. 
This can help us show a lack of last-iterate convergence for other slightly more niche algorithms in the literature that use potential function ideas.
}

We unpack the above statement in a series of comments below.
{\color{red} Vidya: We will consider amending the writing here once all of these extensions have actually been proved. Some of this could also go in a later section.}

\begin{remark}
The result above implies that the outcome of \textit{both} players playing no-regret algorithms with the above properties is last-iterate divergence in the following ``proof-by-contradiction" style reasoning: If last-iterate convergence of \textit{both players} was possible, then the outcome of this interaction would need to have player $2$ converging \textit{almost surely} to NE, thus, remaining arbitrarily close to NE with arbitrarily high probability after enough iterations.
Our result above implies that, then, player $1$ will necessarily diverge as a direct consequence of the stochasticity in the realizations of play of player $2$'s mixed strategy on every round (which is always arbitrarily close to NE).
{\color{red} Vidya: this is intentionally vaguely worded at the moment and will be updated once we have extended our proof argument.}
\end{remark}

\begin{remark}
Our result does not imply last-iterate divergence for \textit{all} no-regret algorithms: we have assumed that the strategies use empirical averages of the other player's plays as a sufficient statistic (along with the round number itself).
However, we subsequently show, in two important extensions of this result, that this reasoning can be slightly modified to show last-iterate divergence for commonly used variations of such strategies.
The first such variation is \textit{optimism}, that has seen success in last-iterate convergence in the \textit{deterministic} variant of repeated interaction, where each player can see the other's mixtures (not just their realizations).
In the actual setting that will occur in repeated interaction, players only observe their opponents' realizations, and we show that all optimistic algorithms will also suffer last-iterate divergence.
{\color{red} Vidya: this is essentially a cosmetic extension}
The second variation that we consider, for completeness, constitutes reductions to \textit{internal-no-regret} algorithms that use a slightly different notion of empirical average as a sufficient statistic.
We show, using very similar arguments to Theorem~\ref{thm:lastiterateconvergence}, that all such algorithms will also diverge in their last iterate.
Thus, the reliance on empirical averages for the players' strategies is more an approximate one than an exact one for the purposes of our proofs.
Our results, in sum, imply that any strategy that could successfully converge in the last-iterate would need to deviate, significantly, from using the empirical averages of past play and use a much stronger recency bias than the one used in typical optimistic variants of Mirror Descent --- whether it is possible to design such algorithms while maintaining the no-regret property is an open question.
\end{remark}

{\color{red} Vidya: We want to use this last remark to say something like this: ``We checked \textit{all} no-regret algorithms, both external and internal, in the literature; and showed that they cannot converge in the last-iterate.}

\mycomment{Let's include another important remark that we restrict our strategies to optimal no-regret, that is with a regret of the order of at most $\sqrt{T}$.}

Putting this reasoning together, our results provide partial, but compelling corroborative evidence for the possibility that the very requirement of no-regret, itself, could preclude last-iterate convergence for either player even in the simplest possible case, which is $2 \times 2$ zero-sum games.
We note that recent work on \textit{smoothly calibrated strategies} (which do not in general satisfy the no-regret property) highlights the possibility of their last-iterate convergence to NE, even for general games.
We discuss this work in more detail in Section~\ref{sec:otheralgorithms}.

\section{Related work}

In this section, we discuss relevant related work to our perspectives on last-iterate convergence/divergence of learning dynamics.

\subsection{Convergence in time averages to equilibrium}

Classical guarantees on convergence to equilibrium, whether Nash or correlated, have been shown on the \textit{time averages} of the players' realizations of strategies.
Several choices of learning dynamics have been considered in the economics(~\cite{brown1951iterative,fudenberg1998learning,foster1997calibrated,hart2000simple,hart2005adaptive}), online learning(~\cite{littlestone1989weighted,freund1999adaptive,kalai2005efficient,blum2007external}) and control theory(~\cite{}) literature.
{\color{red} Vidya: todo, find the appropriate controls literature}
One of the oldest learning dynamics, \textit{fictitious play}(~\cite{brown1951iterative}), involves players best-responding to the empirical average of their opponents' play.
This dynamic has long been known to lead to divergence of the time-average of each player's strategies from NE, even for simple zero-sum games.
Learning dynamics that incorporate explicit randomization, such as multiplicative weights and ``Follow-the-Perturbed Leader" (the former was first conceptualized by Littlestone and Warmuth(~\cite{littlestone1989weighted}); the latter idea goes back to Hannan(~\cite{hannan1957approximation})) have also been considered under the umbrella term of ``adaptive heuristics". 
These have seen more success: the time averages of their updates are known to converge to the NE of a zero-sum game\footnote{In fact, as detailed in (~\cite[Chapter 9]{cesa2006prediction}), this constitutes an alternative proof of the minimax theorem.}.
These are all examples of \textit{no-regret algorithms} --- the idea of no-regret is spiritually related to Blackwell's approachability condition(~\cite{blackwell1956}), and more recently these two notions were shown to be equivalent in a strong sense(~\cite{abernethy2011blackwell}).

In fact, remarkable properties of the time-average of strategies can be shown even in general games, but not to the NE\footnote{In fact, convergence to the NE for a special class of general games is known to be impossible for all uncoupled dynamics(~\cite{hart2003uncoupled}), of which no-regret algorithms form a subset.}.
The notion of no-regret that all of the above algorithms satisfy (called \textit{external} no-regret in the online learning literature) measures the suboptimality of utility with respect to the utility that could have been obtained by playing any single strategy \textit{on all rounds} of the game.
A more refined benchmark, called \textit{internal} no-regret in the online literature(~\cite{blum2007external}), benchmarks utility against the maximal utility obtainable by swapping all instances of a particular pure strategy played with an alternative strategy.
{\color{red} Vidya: slightly hand-wavy explanation of no-internal-regret; read papers again and update}
% It turns out that this is a strictly stronger requirement; all strategies that are no-internal-regret are also no-external-regret, but not vice-versa.
When strategies satisfying the stronger no-internal-regret condition are played against one another, they will converge to the set of correlated equilibria of a general game(~\cite{foster1997calibrated,hart2000simple,hart2005adaptive}).
Note that the time-average of players' strategies are random quantities owing to the randomness in realizations.
Accordingly, the time-average of strategies is shown to converge \textit{almost surely} over this randomness.

\subsection{Recent work on last-iterate convergence and min-max optimization}

As we noted in the introduction, convergence of the time average of the players' realizations of strategies to NE does not imply that their joint distributions used at every round, themselves, converge.
The question of whether such \textit{last-iterate} convergence happens has received recent attention with a surprising result(~\cite{bailey2018multiplicative}): players who use the common no-regret dynamic, exponential weights/Follow-the-Regularized Leader, suffer last-iterate divergence, or convergence to a limit cycle of joint distributions (which averages to the NE).
This chaotic behavior has also been observed in the continuous-time equivalents of these algorithms(~\cite{mertikopoulos2018cycles}).
Spiritually related to this is also the cycling behavior of continuous optimization algorithms such as gradient descent (ascent) when used in \textit{min-max} optimization of a differentiable function that is convex in its first argument and concave in its second argument (e.g.~\cite{mazumdar2018convergence}, but also observed in many other papers).

These algorithmic observations have also received much attention in the ML community, as gradient-descent-ascent is commonly used as an optimization algorithm to train generative adversarial networks, which involves finding the arg-min of an appropriately defined\footnote{In addition to the chaotic algorithmic behavior, several other issues arise in the optimization landscape relating to the limit points of gradient-descent-ascent related to the possible non-convexity/concavity of the objective in GANs.} min-max optimization problem.
The chaotic behavior is usually attributed to specific issues with gradient descent in particular being used as the base algorithm: in particular, \textit{optimistic} variants of gradient descent/ascent, that incorporate a recency bias in their updates, can be shown to remedy the issue and lead to convergence in min-max optimization(~\cite{daskalakis2017training,mertikopoulos2018mirror,liang2018interaction}).

Optimism has also, coincidentally, led to faster convergence of \textit{time-averages} in the game-theoretic settings both for zero-sum and non-zero-sum games(~\cite{rakhlin2013optimization,syrgkanis2015fast}).
Most recently, last-iterate convergence was also shown in the game-theoretic setting for optimistic exponential weights recently(~\cite{daskalakis2018last}).
However, this result made a critical assumption that is unrealistic in repeated interaction: namely, that every player is able to observe her opponent's choice of \textit{mixed strategy} in past rounds, and use this information in her update.
Under this assumption, the evolution of jointly distributed strategies is a \textit{deterministic} dynamical system.
We consider the more realistic, and traditionally considered, setting in which players only use their opponents' \textit{stochastic realizations} drawn from their mixed strategies, constituting a \textit{stochastic} dynamical system\footnote{Note that all of the classical results on convergence of the time averages are stochastic dynamical systems for this reason, the stochasticity arising from realizations of mixed strategies of both players and impacting both the outcomes of current rounds, and future strategies.}.
As we will see shortly, this stochasticity critically matters, and we show that optimistic variants of algorithms no longer converge in the last iterate in the actually realistic setting.
{\color{red} Vidya: weighing in pretty strongly here; we can discuss whether to tone down the language.}
\mycomment{I would like to bring this too in the beginning, say along with the remarks above.
And along with this it would be nice to explain in words the high level idea behind our result -- optimal no-regret requires a minimum level of sensitivity in the strategy of a player towards her opponent's actions, and this sensitivity is strong enough to even pick up the noise in the opponents action and avoid its convergence.
}

% \subsection{Perspectives from min-max optimization: does recency bias help?}

\subsection{Properties of other algorithms of interest (that can suffer linear regret)}\label{sec:otheralgorithms}

A very reasonable question to ask, in the light of our negative results on last-iterate divergence for such a broad class of no-regret algorithms, is whether \textit{any} non-trivial dynamics, whether no-regret or otherwise, can be guaranteed to converge in the last iterate.
In fact, algorithms satisfying a notion of \textit{smoothed calibration} can be shown to converge in precisely this fashion(~\cite{foster2018smooth}).
{\color{red} Vidya: going to write this section later once we understand this paper better. This may also come later in the paper after our main results are stated.}

% {\color{blue} High level question/motivation: Convergence of no-regret strategies. 
% Point to the relevant work in literature and explain their setting in short.
% Our framework and key result/lemma about no-regret learning.
% Natural application to game theory in population games.}


% We consider a scenario where we have two groups each with a large number of players in our population,
% and at any instant two players, one from each group, are chosen at random and made to play a game of matching pennies against each other with player from group 1 playing the role of player 1 and the one from group 2 playing the role of player 2.
% {\color{blue} Give real world examples to motivate this problem. One could think of a general scenario where some $m > 1$ players are grouped randomly and they play some fixed $m$-player normal form game and then the group scatters. Compare this with the literature on Evolutionary games.}
% We can now imagine a strategy for any fixed player in either of the groups to be a function from her past interactions (or histroy of play) to a real number in $[0,1]$ that describes her mixed action in the next game.
% Note that we allow the strategies of the players to be different from each other.
% We will restrict the function from past interactions of any player to depend only on the empirical average of the actions of the opponents that this player has faced till then and the number of games this player has played till then.
% In particular, the above assumption implies that while deciding on the mixed action to play at any instance, the following holds: 
% \begin{inparaenum}[(i)] 
% \item that the players ignore the actions they played until then, and
% \item the players ignore the ordering in the observed actions of the opponents and hence they do not display any recency bias.
% \end{inparaenum}
% The first assumption makes sense because in a large population game it is highly unlikely that any player is going to be paired with the same player again and hence she is going to play myopically and not worry about the implications of her action on the behaviour of her opponent or on the population.
% The second assumption is rather limiting, but note that several known no-regret learning strategies like multiplicative weights update, follow the perturbed leader, satisfy this assumption.
% We will later try to weaken this assumption and allow for recency bias.
% Further, we suppose each of our players to play a no-regret learning strategy (defined shortly).
% For example, if a player had a prior on the distribution of the opponents action, then the best response will be either a pure action 0 or a pure action 1.
% Thus it makes sense to consider a regret with respect to the best of the fixed stategies.
% Given this setting, we will ask ourselves the following question: Can the mixed actions played by the players converge?
% {\color{blue} Relate the above problem with the literature on two player games with multiplicative update rule strategies.}


% {\color{blue} Document structure roughly:

% - no-regret strategy definition

% - uniform no-regret strategy definition

% - rate of no-regret definition

% - implication of this rate on the strategy functions (wiggle result)

% - Sensitivity of the no-regret strategy to random perturbations

% - conclude with implications to population games introduced above
% }

==> tex/monotonicity_proof_orig.tex <==
%!TEX root = ../main_supp.tex

\begin{abstract}
In this supplement, we provide a full proof for the last-iterate divergence conjecture (Conjecture 3.4) under the additional assumption that the strategy functions $\{f_t,g_t\}_{t \geq 1}$ are monotone increasing and decreasing respectively in their arguments.
We also show that the proofs extend to a broad family of algorithms with adaptive step-sizes, which are neither mean-based nor self-agnostic.
All proofs are presented for the matching pennies game for brevity and simplicity, but will easily extend to all $2 \times 2$ competitive games.
\end{abstract}

% \section{Simplified ``warm-up" proof under monotonicity}

% We carry over the entire setup from Section 2 of the paper, and additionally assume that $f_t(\cdot)$ is monotonically \textit{increasing} in its argument for all $t \geq 1$, i.e. $f_t(q) \leq f_t(q')$ for any $q \leq q'$.
% Note that this does not require \textit{strict} monotonicity anywhere, which would be a much stronger assumption.
% This implies a highly simplified \textit{deterministic} statement of fluctuation-sensitivity.
% In particular, Equation (16) (in the proof of Theorem 2) yields the following condition for any mean-based, self-agnostic no-regret algorithm:
% \begin{align}\label{eq:deterministiccondition}
% f_{t_k}\left(\frac{1}{2} + \frac{\beta}{\sqrt{t_k}}\right) \geq \frac{1}{2} + \delta \text{ for all } k \geq 1 ,
% \end{align}

% where $\{t_k\}_{k \geq 1}$ is the sequence that was defined in Proposition 8.
% (This follows because if Equation~\eqref{eq:deterministiccondition} were \textit{not} true, we would get $f_{t_k}(z/t_k) \leq 1/2 + \delta$ for all $z \leq 1/2 + \beta/\sqrt{t_k}$ by monotonicity on $f_t(\cdot)$, which would violate the statement of Equation (16).)
% Applying the monotonicity assumption again gives us
% \begin{align}\label{eq:noregretsensitivity2}
% f_{t_k}(x) \geq \frac{1}{2} + \delta \text{ for all } x \geq \frac{1}{2} + \frac{\beta}{\sqrt{t_k}} \text{ and for all } k \geq 1 .
% \end{align}
% %
% Now, we can get a trivial proof of last-iterate divergence for the ``warm-up" case, i.e. player $2$ already converged to equilibrium ($q_t = 1/2$ for all $t \geq 1$) from the deterministic condition in Equation~\eqref{eq:noregretsensitivity2}.
% This is because
% \begin{align*}
% \bbP\left[\bm{P}_{t_k} \geq \frac{1}{2} + \delta \right] &= \bbP\left[f_{t_k}(\widehat{\bm{Q}}_{t_k-1}) \geq \frac{1}{2} + \delta \right] \\
% &\stackrel{(\mathsf{i})}{\geq} \bbP\left[\widehat{\bm{Q}}_{t_k-1} \geq \frac{1}{2} + \frac{\beta}{\sqrt{t_k}}\right] \\
% &\stackrel{(\mathsf{ii})}{\geq} \frac{1}{2} \cdot \bbP\left[W \geq 2 \beta \right] \text{ where } W \sim \mathcal{N}(0,1) \\
% &= \frac{1}{2} \text{erfc}(2 \beta) := \epsilon(\delta) > 0 \text{ for any } \delta < 1/4 .
% \end{align*}
% %
% Recall that $\bm{P}_{t_k}$ refers to the individual iterates, and $\widehat{\bm{Q}}_{t_k}$ refers to the time-average of iterates.
% Above, inequality $(\mathsf{i})$ follows from Equation~\eqref{eq:noregretsensitivity2} and inequality $(\mathsf{ii})$ follows from the central limit theorem, where $1/2 < 1$ is chosen as an arbitrary constant.
% This completes the proof for the ``warm-up" case.
% \qed

\section{Full proof of last-iterate divergence using martingale CLT}

Finally, we show that Equation~\eqref{eq:noregretsensitivity2} admits a full proof of last-iterate divergence, essentially a proof of Conjecture 3.4, using the martingale CLT.
\begin{proof}
We will adopt the same ``proof-by-contradiction'' structure.
We will show that, if $\bm{Q}_t \to 1/2 \text { a.s.}$, then we need to have
\begin{align*}
\lim_{t \to \infty} \bbP\left[\bm{P}_t \geq \frac{1}{2} + \delta \right] \geq \epsilon(\delta) > 0 \text{ for any } 0 < \delta < 1/4 . 
\end{align*}
%
First, we prove the following claim.
\begin{claim}
$\bm{Q}_t \to 1/2 \text{ a.s. }$ implies that
\begin{align}\label{eq:continuumclosetoNE}
{\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \left\{s \leq t_k: \frac{1}{4} \leq \bm{Q}_s \leq \frac{3}{4}\right\} \Big{|} = 1 \text{ almost surely, }
\end{align}
where $\{t_k\}_{k \geq 1}$ was the deterministic subsequence used in Proposition 8.
\end{claim}
%
Equation~\eqref{eq:continuumclosetoNE} is reminiscent of a convergence condition that is used by~\citet{foster2018smooth}.
We now prove the claim.
\begin{proof}
Let $\Omega$ denote the $\sigma$-algebra induced by $\{\bm{P}_t,\bm{Q}_t\}_{t \geq 1}$ and the strategies $\{f_t(\cdot),g_t(\cdot)\}_{t \geq 1}$.
let $\omega \in \Omega$ denote any realization of this, and $(\bm{P}_t(\omega),\bm{Q}_t(\omega))$ denote the corresponding mixed strategies at time $t$.
Then, $\bm{Q}_t \to 1/2$ a.s. implies that
\begin{align*}
\bbP\left(\omega \in \Omega: \lim_{t \to \infty} \bm{Q}_t(\omega) = 1/2 \right) = 1 .
\end{align*}
%
This directly implies that for any subsequence $\{t_k\}_{k \geq 1}$, we get
\begin{align*}
\bbP\left(\omega \in \Omega: \lim_{k \to \infty} \bm{Q}_{t_k}(\omega) = 1/2 \right) = 1 .
\end{align*}
%
For every $\omega$ such that $\lim_{t \to \infty} \bm{Q}_{t}(\omega) = 1/2$, there exists finite $t_0(\omega)$ such that
\begin{align*}
\bm{Q}_{t}(\omega) \in \left[\frac{1}{4},\frac{3}{4} \right] \text{ for all } t \geq t_0(\omega) .
\end{align*}

Let $k_0(\omega) := \min\{k: t_k \geq t_0(\omega)\}$.
This directly gives us
\begin{align*}
{\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \{s \leq t_k: \frac{1}{4} \leq \bm{Q}_s(\omega) \leq \frac{3}{4}\} \Big{|} \geq {\lim \inf}_{k \to \infty} \frac{t_k - t_{k_0(\omega)})}{t_k} = 1 .
\end{align*}
Thus, we directly get
\begin{align*}
\bbP\left(\omega \in \Omega: {\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \left\{s \leq t_k: \frac{1}{4} \leq \bm{Q}_s(\omega) \leq \frac{3}{4}\right\} \Big{|} = 1 \right) = 1 ,
\end{align*}
which completes the proof.
\end{proof}
%
Thus, we have proved our claim.
As a direct consequence of the above claim, we have
\begin{align}\label{eq:variancebound}
{\lim \inf}_{t \to \infty} \frac{1}{t} \sum_{s=1}^t \bm{Q}_s(1 - \bm{Q}_s) \geq \frac{3}{16} \text{ almost surely. } 
\end{align}
%
We consider the filtration $\{\mathcal{F}_t := (\bm{I}_s,\bm{J}_s)_{s=1}^{t-1}\}_{t \geq 1}$, and the stochastic process $\{\bm{D}_t := \bm{Z}_t - \bm{Z}_{t-1} - \bm{Q}_t\}_{t \geq 1}$.
Recall that we had defined $\bm{Z}_t := \sum_{s=1}^t \bm{J}_t$, where $\bm{J}_t \sim \text{Ber}(\bm{Q}_t)$.
We observe the following properties of the stochastic process $\{\bm{D}_t\}_{t \geq 1}$:
\begin{enumerate}
\item $\bm{D}_t$ is a martingale difference sequence with respect to the filtration $\mathcal{F}_{t-1}$. 
This is a direct consequence of $\bm{Q}_t$ being a \textit{deterministic} function of $\mathcal{F}_{t-1}$.
\item $|\bm{D}_t| \leq 1$.
\item The sum of conditional variances diverges to $\infty$.
In other words, we have
\begin{align*}
\sigma_t^2 := \bbE\left[\bm{D}_t^2 | \mathcal{F}_{t-1}\right] &= \bbE\left[(\bm{J}_t - \bm{Q}_t)^2 | \mathcal{F}_{t-1}\right] \\
&= \bm{Q}_t(1 - \bm{Q}_t) ,
\end{align*}
and from Equation~\eqref{eq:variancebound} it is clear that ${\lim \inf}_{t \to \infty} \sum_{s=1}^t \sigma_s^2 = \infty$ a.s.
% \vidyacomment{In fact, the (asymptotic) rate of divergence to infinity is linear as a consequence of Equation~\eqref{eq:variancebound}; we will use this shortly.}
\end{enumerate}


As a consequence of these properties, we can apply the martingale central limit theorem~\citep{hall2014martingale} in the following form:

\begin{theorem}[Martingale CLT,~\citep{hall2014martingale}]\label{thm:martingaleCLT}
Let $\{\bm{D}_t\}_{t \geq 1}$ be a martingale difference sequence with respect to the filtration $\mathcal{F}_{t-1}$ such that $|\bm{D}_t| \leq 1$.
Further, let $\{\sigma_t^2 := \bbE\left[\bm{D}_t^2 | \mathcal{F}_{t-1}\right]\}_{t \geq 1}$ denote the conditional variance sequence with the property that $\sum_{t=1}^{\infty} \sigma_t^2$ diverges to infinity almost surely.
Then, we have
\begin{align}\label{eq:martingaleCLT}
\frac{\sum_{s=1}^t \bm{D}_s}{\sqrt{\sum_{s=1}^t \sigma_s^2}} \to \bm{Z} \sim \mathcal{N}(0,1) .
\end{align}
\end{theorem}
%
Note that Equation~\eqref{eq:martingaleCLT} directly implies
\begin{align}\label{eq:martingaleCLTsubsequence}
\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{\sum_{s=1}^{t_k} \sigma_s^2}} \to \bm{Z} \sim \mathcal{N}(0,1) .
\end{align}
%
for any deterministic subsequence $\{t_k\}_{k \geq 1}$.
From Proposition 8, we get
\begin{align*}
{\lim \inf}_{k \to \infty} \bbP\left( \bm{P}_{t_k} \geq \frac{1}{2} + \delta \right) &\geq \lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - 1/2) \geq \beta \right) \\
&\stackrel{\mathsf{(i)}}{\geq} \lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k}) \geq \beta' \right)
\end{align*}
%
Inequality $(\mathsf{i})$ follows because of the statement made in Appendix C of the main paper, which is
\begin{align*}
\overline{\bm{Q}}_t \geq \frac{1}{2} - \frac{C}{\sqrt{t}} \text{ pointwise, for all } t \geq 1 
\end{align*}
%
for some bounded constant $C > 0$.
Above, we denote $\beta' := \beta + C$.
%
Now, note that for any $k \geq 1$, we have $\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{t_k}} = \frac{1}{\sqrt{t_k}}\left( \bm{Z}_{t_k} - \sum_{s=1}^{t_k} \bm{Q}_s \right) = \sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k})$.
Therefore, we get
\begin{align*}
\lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k}) \geq \beta' \right) &= \lim_{k \to \infty} \bbP\left( \frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{t_k}} \geq \beta' \right) \\
&\stackrel{\mathsf{(i)}}{\geq} \lim_{k \to \infty} \bbP\left(\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{\sum_{s=1}^{t_k} \bm{Q}_s(1 - \bm{Q}_s)}}\geq \frac{16\beta'}{3} \right) \\
&\stackrel{\mathsf{(ii)}}{\geq} \text{erfc}(c) > 0 .
\end{align*}
%
where $c := \frac{16\beta'}{3}$.
Inequality $(\mathsf{i})$ uses Equation~\eqref{eq:continuumclosetoNE}, and inequality $(\mathsf{ii})$ uses the martingale CLT on the subsequence $\{t_k\}_{k \geq 1}$ (as described in Equation~\eqref{eq:martingaleCLTsubsequence}.
% \vidyacomment{Note that both of these are applied as almost sure convergence statements on the deterministic subsequence $\{s_t\}_{t \geq 1}$, which is valid because a) the convergence is almost sure, and b) the subsequence is deterministic and fixed in advance.} 
Thus, we have shown that if the last iterate of player $2$ were assumed to converge, the last iterate of player $1$ could not converge (in fact, even in probabality).
This completes our \textit{proof-by-contradiction}: at least one of the players cannot converge almost surely to NE.
\end{proof}

\section{Extended proof for Hedge with adaptive step sizes}

In this section, we present a very brief proof of Conjecture 3.4 for all known variants of Hedge with adaptive step sizes, i.e. 
\begin{align*}
\bm{P}_t &= \frac{\exp\{\eta_t \bm{Z}_{t-1} \}}{\exp\{\eta_t \bm{Z}_{t-1} \} + \exp\{\eta_t (t - 1 - \bm{Z}_{t-1})\}} ,
\end{align*}

where $\eta_t := \eta_t(\mathcal{F}_{t-1})$.
This includes algorithms that achieve variation-based bounds~\cite{hazan2010extracting}, algorithms that adapt between adversity and stochasticity~\cite{cesa2007improved,erven2011adaptive}, and learning on predictable sequences~\cite{rakhlin2013online,rakhlin2013optimization}.
The adaptive learning rate can be set via the ubiquitous ``doubling-trick"~\cite{cesa2007improved,hazan2010extracting} or in a more continuous manner~\cite{erven2011adaptive,rakhlin2013online,rakhlin2013optimization}.
% \vidyacomment{TODO: fill in such algorithms; Rakhlin-Sridharan algorithm also needs to be added.}
Either way, none of these algorithms do not satisfy either the mean-based property, and some of them (most notably AdaHedge~\cite{cesa2007improved,erven2011adaptive}) do not satisfy even the self-agnostic property.
This is because in general, the learning rate function $\eta_t(\mathcal{F}_{t-1})$ will depend in some non-linear way on $\{\bm{P}_s,\bm{Q}_s,\bm{I}_s,\bm{J}_s\}_{s=1}^{t-1}$.

In spite of this, we can prove last-iterate divergence for these algorithms.
We critically use the following property that is shared by all such adaptive algorithms: for some universal constant $C > 0$, we have
\begin{align*}
\eta_t \geq \frac{C}{\sqrt{t}} \text{ pointwise. }
\end{align*}

This property is usually used to prove that adaptive Hedge algorithms retain the $\mathcal{O}(\sqrt{t})$ regret guarantee in the worst case (but can get faster rates under more favorable conditions).
For a given round $t$, we define $\bm{Z}_{t-1}$ as above, and further define
\begin{align*}
\bm{P}_{t,\mathsf{Hedge}} := f_{t,C}(\widehat{\bm{Q}}_{t-1}) := \frac{\exp\{C \sqrt{t} \widehat{\bm{Q}}_{t-1} \}}{\exp\{C \sqrt{t} \widehat{\bm{Q}}_{t-1} \} + \exp\{C \sqrt{t} (1 - \widehat{\bm{Q}}_{t-1})\}}
\end{align*}

as the counterfactual iterate that would have been generated if the algorithm switched to Hedge with learning rate $\eta_t = C/\sqrt{t}$ at round $t$, and we note that $|2\bm{P}_{t} - 1| \geq |2\bm{P}_{t,\mathsf{Hedge}} - 1|$.
Clearly, $\{f_{t,C}(\cdot)\}_{t \geq 1}$ is a mean-based and self-agnostic strategy, and so it satisfies the deterministic statement of Equation~\eqref{eq:noregretsensitivity2} for all $t := t_k$.
That is, we have for every $k \geq 1$,
\begin{align*}
f_{t_k, C}(x) \geq \frac{1}{2} + \delta \text{ for all } x \geq \frac{1}{2} + \frac{\beta}{\sqrt{t_k}} \text{ and for all } k \geq 1 .
\end{align*}

Therefore, we get for any $k \geq 1$,
\begin{align*}
\bbP\left(\bm{P}_{t_k} \geq \frac{1}{2} + \delta \right) \geq \bbP\left(\bm{P}_{t_k,\mathsf{Hedge}} \geq \frac{1}{2} + \delta \right) ,
\end{align*}

and the proof directly follows by lower bounding the right hand side.
This completes the proof of last-iterate divergence for Hedge with adaptive step sizes.
\qed

\begin{remark}
Note that the above proof did not use any details about the adaptive step sizes or the fact that the underlying framework was the Hedge algorithm.
The only necessary property is that the iterates stochastically dominate the iterates of an equivalent mean-based no-regret algorithm.
Thus, this proof idea would be more broadly applicable to any no-regret algorithm that can be ``reduced" to a mean-based, self-agnostic algorithm in this sense.
\end{remark}



==> tex/proof_martingale.tex <==
\begin{proof}
We will use the approach of \textit{proof-by-contradiction}.
Suppose that we in fact have $(\bm{P}_t \to p^*, \bm{Q}_t \to q^*) \text{ a.s.}$.
Note that this trivially implies that $\bm{Q}_t \to q^* \text{ a.s.}$
To complete the proof by contradiction, we will show that if $\bm{Q}_t \to q^* \text { a.s.}$, then we need to have
\begin{align*}
\lim_{t \to \infty} \bbP\left[\bm{P}_t \geq p^* + \delta \right] \geq \epsilon(\delta) > 0 \text{ for any } 0 < \delta < 1/4 . 
\end{align*}
%
Our first critical ingredient is the following claim, which implies sufficient stochasticity in the iterates under the assumed almost sure convergence of the mixed strategies of player $2$.
\begin{claim}
$\bm{Q}_t \to q^* \text{ a.s. }$ implies that
\begin{align}\label{eq:continuumclosetoNE}
{\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \left\{s \leq t_k: \frac{q^*}{2} \leq \bm{Q}_s \leq \frac{q^* + 1}{2}\right\} \Big{|} = 1 \text{ almost surely, }
\end{align}
for any deterministic sub-sequence $\{t_k\}_{k \geq 1}$.
\end{claim}
%
Equation~\eqref{eq:continuumclosetoNE} is reminiscent of a convergence condition that is used by~\citet{foster2018smooth} for ``smoothly calibrated'' strategies.
We now prove the claim.
\begin{proof}
Let $\Omega$ denote the $\sigma$-algebra induced by $\{\bm{P}_t,\bm{Q}_t\}_{t \geq 1}$ and the strategies $\{f_t(\cdot),g_t(\cdot)\}_{t \geq 1}$.
Let $\omega \in \Omega$ denote any realization of this, and $(\bm{P}_t(\omega),\bm{Q}_t(\omega))$ denote the corresponding mixed strategies at time $t$.
Then, $\bm{Q}_t \to q^*$ a.s. implies that
\begin{align*}
\bbP\left(\omega \in \Omega: \lim_{t \to \infty} \bm{Q}_t(\omega) = q^* \right) = 1 .
\end{align*}
%
This directly implies that for any subsequence $\{t_k\}_{k \geq 1}$, we get
\begin{align*}
\bbP\left(\omega \in \Omega: \lim_{k \to \infty} \bm{Q}_{t_k}(\omega) = q^* \right) = 1 .
\end{align*}
%
This implies, by the definition of a limit, that for every $\omega$ such that $\lim_{t \to \infty} \bm{Q}_{t}(\omega) = q^*$, there exists finite $t_0(\omega)$ such that
\begin{align*}
\bm{Q}_{t}(\omega) \in \left[\frac{q^*}{2},\frac{q^* + 1}{2} \right] \text{ for all } t \geq t_0(\omega) .
\end{align*}

Let $k_0(\omega) := \min\{k: t_k \geq t_0(\omega)\}$.
This directly gives us
\begin{align*}
{\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \left\{s \leq t_k: \frac{q^*}{2} \leq \bm{Q}_s(\omega) \leq \frac{q^* + 1}{2}\right\} \Big{|} \geq {\lim \inf}_{k \to \infty} \frac{t_k - t_{k_0(\omega)}}{t_k} = 1 .
\end{align*}
Thus, we directly get
\begin{align*}
\bbP\left(\omega \in \Omega: {\lim \inf}_{k \to \infty} \frac{1}{t_k} \Big{|} \left\{s \leq t_k: \frac{q^*}{2} \leq \bm{Q}_s(\omega) \leq \frac{q^* + 1}{2}\right\} \Big{|} = 1 \right) = 1 ,
\end{align*}
which completes the proof.
\end{proof}
%
Thus, we have proved our claim.
As a direct consequence of the above claim, we have
\begin{align}\label{eq:variancebound}
{\lim \inf}_{t \to \infty} \frac{1}{t} \sum_{s=1}^t \bm{Q}_s(1 - \bm{Q}_s) \geq \min\left\{\frac{q^*(2 - q^*)}{4},\frac{(1 + q^*)(1 - q^*)}{4} \right\} := \gamma(q^*) \text{ a.s. } 
\end{align}
%
We consider the filtration $\{\mathcal{F}_t := (\bm{I}_s,\bm{J}_s)_{s=1}^{t-1}\}_{t \geq 1}$, and the stochastic process $\{\bm{D}_t := \bm{Z}_t - \bm{Z}_{t-1} - \bm{Q}_t\}_{t \geq 1}$.
Recall that we had defined $\bm{Z}_t := \sum_{s=1}^t \bm{J}_t$, where $\bm{J}_t \sim \text{Ber}(\bm{Q}_t)$.
We observe the following properties of the stochastic process $\{\bm{D}_t\}_{t \geq 1}$:
\begin{enumerate}
\item $\bm{D}_t$ is a martingale difference sequence with respect to the filtration $\mathcal{F}_{t-1}$. 
This is a direct consequence of $\bm{Q}_t$ being a \textit{deterministic} function of $\mathcal{F}_{t-1}$.
\item $|\bm{D}_t| \leq 1$.
\item Note that because $0 < q^* < 1$, we have $\gamma(q^*) > 0$.
Therefore, the sum of conditional variances diverges to $\infty$.
In other words, we have
\begin{align*}
\sigma_t^2 := \bbE\left[\bm{D}_t^2 | \mathcal{F}_{t-1}\right] &= \bbE\left[(\bm{J}_t - \bm{Q}_t)^2 | \mathcal{F}_{t-1}\right] \\
&= \bm{Q}_t(1 - \bm{Q}_t) \geq \gamma(q^*)
\end{align*}
and from Equation~\eqref{eq:variancebound} it is clear that ${\lim \inf}_{t \to \infty} \sum_{s=1}^t \sigma_s^2 = \infty$ a.s.
% \vidyacomment{In fact, the (asymptotic) rate of divergence to infinity is linear as a consequence of Equation~\eqref{eq:variancebound}; we will use this shortly.}
\end{enumerate}


As a consequence of these properties, we can apply the martingale central limit theorem~\citep{hall2014martingale} in the following form:

\begin{theorem}[Martingale CLT,~\citep{hall2014martingale}]\label{thm:martingaleCLT}
Let $\{\bm{D}_t\}_{t \geq 1}$ be a martingale difference sequence with respect to the filtration $\mathcal{F}_{t-1}$ such that $|\bm{D}_t| \leq 1$.
Further, let $\{\sigma_t^2 := \bbE\left[\bm{D}_t^2 | \mathcal{F}_{t-1}\right]\}_{t \geq 1}$ denote the conditional variance sequence with the property that $\sum_{t=1}^{\infty} \sigma_t^2$ diverges to infinity almost surely.
Then, we have
\begin{align}\label{eq:martingaleCLT}
\frac{\sum_{s=1}^t \bm{D}_s}{\sqrt{\sum_{s=1}^t \sigma_s^2}} \to \bm{Z} \sim \mathcal{N}(0,1) .
\end{align}
\end{theorem}
%
Note that Equation~\eqref{eq:martingaleCLT} directly implies
\begin{align}\label{eq:martingaleCLTsubsequence}
\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{\sum_{s=1}^{t_k} \sigma_s^2}} \to \bm{Z} \sim \mathcal{N}(0,1) .
\end{align}
%
for any deterministic subsequence $\{t_k\}_{k \geq 1}$.
Further, note that for any $k \geq 1$, we have
\begin{align*}
\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{t_k}} = \frac{1}{\sqrt{t_k}}\left( \bm{Z}_{t_k} - \sum_{s=1}^{t_k} \bm{Q}_s \right) = \sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k}).
\end{align*}
%
Consequently, we have for any $\beta' > 0$, 
\begin{align*}
\lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k}) \geq \beta' \right) &= \lim_{k \to \infty} \bbP\left( \frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{t_k}} \geq \beta' \right) \\
&\stackrel{\mathsf{(i)}}{\geq} \lim_{k \to \infty} \bbP\left(\frac{\sum_{s=1}^{t_k} \bm{D}_s}{\sqrt{\sum_{s=1}^{t_k} \bm{Q}_s(1 - \bm{Q}_s)}}\geq \frac{\beta'}{\gamma(q^*)} \right) \\
&\stackrel{\mathsf{(ii)}}{\geq} \text{erfc}\left(\frac{\beta'}{\gamma(q^*)}\right) > 0 .
\end{align*}
%
% where $c := \frac{16\beta'}{3}$.
Above, inequality $(\mathsf{i})$ uses Equation~\eqref{eq:continuumclosetoNE}, and inequality $(\mathsf{ii})$ uses the martingale CLT on the subsequence $\{t_k\}_{k \geq 1}$ (as described in Equation~\eqref{eq:martingaleCLTsubsequence}.

Our next critical observation is a fundamental, classically known~\cite{freund1999adaptive} property of the \textit{average} iterates arising as a consequence of \textit{both} players using no-regret algorithms.
This is that there exists a universal constant $C$ such that
\begin{align*}
\overline{\bm{Q}}_t \geq q^* - \frac{C}{\sqrt{t}} \text{ pointwise, for all } t \geq 1.
\end{align*}
\vidyacomment{TODO: link to appropriate appendix where full proof is provided, state as lemma in main text}
Selecting $\beta' := \beta + C$ for any $\beta > 0$, we then get
\begin{align}\label{eq:effectiveCLT}
\lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - q^*) \geq \beta \right) \geq \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - \overline{\bm{Q}}_{t_k}) \geq \beta' \right) \geq \text{erfc}\left(\frac{\beta + C}{\gamma(q^*)}\right) > 0.
\end{align}
%
Consequently, we can use Equation~\eqref{eq:effectiveCLT} to complete the proof-by-contradiction of Theorem~\ref{thm:lastiteratedivergence}.
In particular, we follow an identical series of steps to the proof of Theorem~\ref{thm:warmup} to show that if $(\bm{P}_t, \bm{Q}_t) \to (p^*,q^*) \text{a.s.}$, we need to have
\begin{align*}
\lim_{k \to \infty} \bbP[\bm{P}_{t_k} \geq p^* + \delta] &\geq \lim_{k \to \infty} \bbP\left(\sqrt{t_k} (\widehat{\bm{Q}}_{t_k} - q^*) \geq \beta \right) \geq \text{erfc}\left(\frac{\beta + C}{\gamma(q^*)}\right) > 0,
\end{align*}
%
where $\beta > 0$ is chosen just as in the proof of Theorem~\ref{thm:warmup}.
This provides the desired contradiction.
% \vidyacomment{The proof after Equation~\eqref{eq:effectiveCLT} has been shown, is exactly identical to the warm-up proof. The proof is exactly identical until Equation (3.17) and the only change is in the constants there-after based on $\beta' \to \beta$. So I am not sure whether to write out the details or not.}
Ultimately, we have shown that if the last iterate of player $2$ were assumed to converge, the last iterate of player $1$ could not converge (in fact, even in probability).
This completes our \textit{proof-by-contradiction}: at least one of the players cannot converge almost surely to NE.
\end{proof}

==> tex/proof_warmup_general.tex <==
%%%%VM: This is currently the ``warm-up'' proof that does not use monotonicity, and will be used in the appendix.
\begin{proof}{}

We start by defining some notation pertinent to mean-based strategies.
Let $\bm{Z_t} \sim \text{Binomial}(t, q^*)$, for $t \geq 1$.
Let $\bm{Z''_{t, s}} \sim \bm{Z_{t-s}} + s$ and $\bm{Q''_{t, s}} = \bm{Z''_{t, s}}/t$, for $0 \leq s \leq t$, $t \geq 1$.
Let $\{(t_k, s_k)\}_{k \geq 1}$ be an infinite sequence and $0 < \delta < (1 - p^*)/3$ as in Proposition~\ref{prop:noregretsensitivity}.
Thus, for every $k \geq 1$, we have
\begin{align*}
    \bm{Q''_{t_k, s_k}} \overset{d}{=} \frac{1}{t} \sum_{s = 1}^t \bm{J'_t(k)},
\end{align*}
where $\overset{d}{=}$ denotes that the two random variables are identical in distribution, and $\bm{J_t'(k)}$ are random variables as defined in Proposition~\ref{prop:noregretsensitivity}.
We thus have
\begin{equation}
    0 < s_k \leq \alpha (t_k)^{1/2}, \text{ for all } k \geq 1,
\end{equation}
and
\begin{align}
\mathbb{E}\left[f_{t_k}\left(\bm{Q''_{t_k, s_k}}\right)\right] \geq p^* + 2\delta, \text{ for all } k \geq 1 ,
\end{align}


Consider the random variable $\bm{Y} := 1 - f_{t_k}(\bm{\widehat{Q}''_{t_k, s_k}})$.
Since the range of $f_t$ is always $[0,1]$, we have $\bm{Y} \geq 0$.
Thus, we have $\mathbb{E}[\bm{Y}] \leq 1 - (p^* + 2\delta) = (1 - p^*) - 2\delta$.
By Markov's inequality, we have
\[
 \bbP\l(\bm{Y} \geq (1 - p^*) - \delta\r) \leq \frac{(1 - p^*) - 2\delta}{(1 - p^*) - \delta}.   
\]
Thus, we get
\begin{equation}
\label{eq: prob_Qt_lowerbdd}
     \bbP\l(f_{t_k}\l(\bm{\widehat{Q}''_{t_k, s_k}}\r) > p^* + \delta\r) \geq \epsilon_0,
\end{equation}
where we define $\epsilon_0 := {\delta}/{((1 - p^*) - \delta)}$.
Note that $0 < \epsilon_0 < 1/2$ (because we had defined $0 < \delta < (1 - p^*)/3$).
By the central limit theorem, we know that 
\[
     \lim_{t \to \infty} \bbP\l(\bm{\widehat{Q}_{t}} > q^* + \frac{\gamma}{\sqrt{t}}  \r) = 1 - \Phi\left(\frac{\gamma}{\sqrt{q^*(1-q^*)}}\right),
 \] 

 where $\Phi(\cdot)$ is the cumulative distribution function of the standard normal distribution.
 Since the function $\Phi(\cdot) : \bbR \to (0,1)$ in continuous, strictly increasing, $\Phi(0) = 1/2$, and $\lim_{x \to \infty} \Phi(x) = 1$,
 we know that
there exists $\gamma_0 > 0$ such that $1 - \Phi(\gamma_0/\sqrt{q^*(1-q^*)}) = \epsilon_0/4$ (note that $\epsilon_0/4 < 1/2)$.
Hence there exists $T_1'(\epsilon_0) > 1$ such that
\[
     \bbP\l(\bm{\widehat{Q}_{t}} > q^* + \frac{\gamma_0}{\sqrt{t}}  \r) \leq (1 - \phi(\gamma_0)) + \frac{\epsilon_0}{4} \leq \frac{\epsilon_0}{2},
 \] 
 for all $t \geq T_1'(\epsilon_0)$.
 
Now, observe that
\[
    t_k\bm{\widehat{Q}''_{t_k, s_k}} \overset{d}{=} (t_k - s_k) \bm{\widehat{Q}_{t_k - s_k}} + s_k.
\]
Since $t_k - s_k \to \infty$ as $k \to \infty$,
there exists a $k_1 > 1$ such that 
 \[
     \bbP \l(t_k \bm{\widehat{Q}''_{t_k, s_k} } > q^*(t_k - s_k) + s_k + \gamma_0 \sqrt{t_k - s_k}  \r) \leq \frac{\epsilon_0}{2},
 \]
 for all $k \geq k_1$.
% 
 Using the bound $s_k \leq \alpha \sqrt{t_k}$, we get
 \begin{equation}
 \label{eq: prob_tail_lowerbdd}
     \bbP \l(\bm{Z''_{t_k, s_k}} > q^* \cdot t_k + \beta \sqrt{t_k} \r) \leq \frac{\epsilon_0}{2},
 \end{equation}
for all $k \geq k_1$, where $\beta := \alpha + \gamma_0$.
From the union bound and Equations~\eqref{eq: prob_Qt_lowerbdd} and \eqref{eq: prob_tail_lowerbdd}, we get
\begin{equation}
\label{eq: prob_markov_tailcut_bdd}
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}''_{t_k, s_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z''_{t_k, s_k}} \leq q^* \cdot t_k + \beta \sqrt{t_k} \r) \geq \frac{\epsilon_0}{2}.
\end{equation}

Recall that we defined the opponent sequence $\{\bm{J_t}\}_{t \geq 1}$ to be an i.i.d. sequence of \newline Bernoulli($q^*$) random variables.
Note that $\bm{Z_t} \overset{d}{=} t \bm{\widehat{Q}_{t}} $, and by definition $\bm{Z''_{t,s}} \geq s$ point-wise.
We denote $\beta_0 := \beta/q^*$.
Note that $q^* t + \beta \sqrt{t} = q^* (t + \beta_0\sqrt{t})$ for any $t$.
Now, we show that
    \begin{equation}
    \label{eq: prob_ratio_lower_bdd}
        \min_{s \leq z \leq q^*(t + \beta_0 \sqrt{t}) }  \; \frac{\bbP(\bm{Z_t} = z)}{\bbP(\bm{Z''_{t,s}} = z)} \geq (1 + \beta_0)^{-\alpha},
    \end{equation}
for all $0 < s \leq \alpha \sqrt{t}$, $t \geq 1$.
Indeed, we have,
    \begin{align*}
        \frac{\bbP(\bm{Z_t} = z)}{\bbP(\bm{Z''_{t,s}} = z)} 
        &= \frac{\binom{t}{z}(q^*)^z (1 - q^*)^{t - z}}{\binom{t-s}{z-s}(q^*)^{z-s} (1 - q^*)^{t - z}}
        = \frac{t}{z} \cdot \frac{t-1}{z-1} \cdots \frac{t-s+1}{z-s+1} \cdot (q^*)^s\\
        &\geq \l(\frac{q^*t}{z}\r)^s
        \geq \l(\frac{t}{t + \beta_0 \sqrt{t}}\r)^{\alpha \sqrt{t}}\\
        &\geq (1 + \beta_0)^{-\alpha} > 0,
    \end{align*}
where the first inequality follows from $z \leq t$ and therefore $\frac{t - \ell}{z - \ell}$ is increasing in $\ell$, and the last inequality follows from the fact that
    \[
        \l(\frac{t + \beta_0 \sqrt{t}}{t}\r)^{\alpha \sqrt{t}} = \l(1 + \frac{\beta_0}{\sqrt{t}}\r)^{\alpha \sqrt{t}} \leq (1 + \beta_0)^{\alpha}.
    \]
    (Note that the function $(1 + \beta_0/x)^{\alpha x}$ is decreasing in $x$ for $x \geq 1$.)

We are now ready to complete our proof via a simple ``change-of-measure" argument and the above lower bound on the ratio of the probability mass functions.
From Equations~\eqref{eq: prob_markov_tailcut_bdd} and \eqref{eq: prob_ratio_lower_bdd} and the law of total probability, we get
\begin{align*}
    &\bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z_{t_k}} \leq q^* \cdot t_k + \beta \sqrt{t_k} \r) \\
    &\geq \sum_{z=s_k}^{q^* \cdot t_k + \beta \sqrt{t_k}} \bbP \l(\bm{Z_{t_k}} = z\r) \cdot \mathbb{I}\left[f_{t_k}\l(\frac{z}{t_{k}}\r) \geq p^* + \delta\right]\\
    &\geq (1 + \beta_0)^{-\alpha} \cdot \sum_{z=s_k}^{q^* \cdot t_k + \beta\sqrt{t_k}} \bbP \l(\bm{Z''_{t_k,s_k}} = z\r) \cdot \mathbb{I}\left[f_{t_k}\l(\frac{z}{t_{k}}\r) \geq p^* + \delta\right] \\
    &= (1 + \beta_0)^{-\alpha} \cdot \bbP \l(f_{t_k} \l(\frac{\bm{{Z''}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z''_{t_k}} \leq q^* \cdot t_k + \beta \sqrt{t_k} \r) \\
    &\geq \frac{\epsilon_0}{2} (1+\beta_0)^{-\alpha},
\end{align*}
and hence
\[
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta\r) \geq \frac{\epsilon_0}{2} (1+\beta_0)^{-\alpha}, 
\]
for $k \geq k_1$.
Since $\bm{P_{t_k}} \overset{d}{=} f_{t_k}(\bm{\widehat{Q}_{t_k}})$, taking $\epsilon := (\epsilon_0/2) (1+\beta_0)^{-\alpha}$, we get
 \begin{align*}
    \bbP\left[\bm{P_{t_k}} \geq p^* + \delta \right] \geq \epsilon,
    \end{align*}
    for all $k \geq k_1$.
    This implies Equation~\eqref{eq: liminf_prob_dev_response} and completes the proof of Theorem~\ref{thm:warmup}.
\end{proof}

==> tex/result_noregret.tex <==
%!TEX root = ../main.tex

\section{Main results}\label{sec:results}

In this section, we use the above assumptions to prove, in a series of steps, that the limiting mixed strategies as an outcome of both players using self-agnostic, mean-based, optimal no regret learning \textit{diverge}.
We start by proving a condition that any self-agnostic, optimal no-regret strategy necessarily satisfies (regardless of whether it is mean-based or not).
As described in Section~\ref{sec: intro}, this condition is described as sensitivity to \textit{fluctuations} in the time-average of the opponent strategy, and is detailed below.

\begin{figure}
    \centering
        \includegraphics[width=0.8\textwidth]{./Figures/sensitivity_figure_proof_2}
    \caption{Response of player $1$, who is using the multiplicative weights algorithm with learning rate $\eta = 1/\sqrt{t}$, against player $2$ who uses the randomized sequence in Equation~\eqref{eq:randomsequence}.
    The blue line plots the time-averages of player $2$, i.e. $\{\bm{\widehat Q_t}\}_{t \geq 1}$, and the red line plots the iterates of player $1$, i.e. $\{\bm P_t\}_{t \geq 1}$.
    Note that the $y$-axis of the figure is on linear scale, so the fluctuation in the time-averages of player $2$ is not visible.
    }\label{fig:sensitivity_figure_proof}
\end{figure}

\begin{proposition}\label{prop:noregretsensitivity}
For any self-agnostic repeated game strategy $\{f_t\}_{t \geq 1}$ used by player $1$ that is uniformly no-regret with a rate of $(r,c)$ 
(where $1/2 \leq r < 1$)
, and any $0 < \delta < (1 -p^*)/3$, there exists a positive constant $\alpha$ and an infinite sequence of integer tuples $\{(t_k,s_k)\}_{k \geq 1}$ such that
\begin{equation}
\label{eq:sensitivitymargin}
    0 < s_k \leq \alpha (t_k)^{r}, \text{ for all } k \geq 1,
\end{equation}
and
\begin{align}\label{eq:sensitivitycondition}
\mathbb{E}\left[f_{t_k}\left(\bm{(J'(k))^{t_k}}\right)\right] \geq p^* + 2\delta, \text{ for all } k \geq 1 ,
\end{align}
where the expectation is over the random sequence $\bm{(J'(k))^{t_k}} := \{\bm{J'_s(k)}\}_{s=1}^{t_k}$ defined as below:
\begin{align}\label{eq:randomsequence}
\bm{J'_s(k)} = \begin{cases}
\bm{J^*_s} \text{ i.i.d. } \sim \text{Bernoulli}(q^*), \text{ if } 1 \leq s \leq t_k - s_k, \\
1 \text{ otherwise. }
\end{cases}
\end{align}
\end{proposition}

In particular, if the self-agnostic repeated game strategy $\{f_t\}_{t \geq 1}$ is \textit{optimally} uniformly no-regret i.e. $r = 1/2$, then condition~\ref{eq:sensitivitymargin} would be
\[
   0 < s_k \leq \alpha \sqrt{t_k}, \text{ for all } k \geq 1. 
\]
For this case, Figure~\ref{fig:sensitivity_figure_proof} shows player $1$'s response, when she uses the multiplicative weight algorithm, to an opponent who plays the random sequence as defined in Equation~\eqref{eq:randomsequence}.
The game that is played is the matching pennies game, which is a zero-sum game with $G(0,0) = G(1,1) = 1$ and $G(0,1) = G(1,0) = 1$.
Her strategy, averaged over player $2$'s realizations, is shown to deviate sizably from the NE of the matching pennies game, $p^* = 0.5$.

This case is important because, even if player $2$ remained close to her equilibrium mixed strategy $q^*$ (as is \textit{necessary} in any hypothetical scenario of last-iterate convergence), there is a non-trivial probability of player $2$'s empirical average deviating from $q^*$ by a number on the order of $1/\sqrt{t}$ at step $t$.
The sensitivity in an optimal no-regret strategy to pick deviations of this order will allow us to show the non-convergence of player $1$'s mixed strategies in the subsequent Sections~\ref{sec:warmup},~\ref{sec:lastiteratedivergence} and~\ref{sec:optimism}.

\proof{Proof.}
Recall that by the competitive $2 \times 2$ game assumption, we have $G(0,1) < G(1,1)$.
Thus, for any $0 \leq p < 1$, we have $G(p,1) < G(1,1)$.
Consider $\{f_t\}_{t \geq 1}$ to be any self-agnostic uniformly no-regret strategy with a no-regret rate of $(r,c)$.
We note that for any $t$, and any sequence $\{J_s\}_{s=1}^t$, we have 
$$\max_{i \in \{0,1\}} \sum_{s=1}^t G(i,J_s) = t \cdot \max\{G(0,\widehat Q_t), G(1,\widehat Q_t)\}.$$
%
Thus, for $c' > c$, there exists a sufficiently large $t_0$ such that for all $t \geq t_0$, we have
\begin{equation}
\label{eq: suff_large_no_regret}
    \frac{1}{t^{r}} \l[t \cdot \max\{G(0,\widehat Q_t), G(1,\widehat Q_t)\} - \sum_{s = 1}^t G(f_s((J)^{s-1}), J_s)) \r] \leq c',
\end{equation}
for any sequence $\{J_s\}_{s = 1}^t$.

Recall that $R^*$ denotes the Nash equilibrium payoff of player $1$.
Because the equilibrium $(p^*,q^*)$ is strictly mixed, we have $R^* = G(p^*,q^*) = G(p^*, 1) < G(1,1)$.
Let $0 < \delta < \frac{(1 - p^*)}{3} = \frac{(G(1,1) - R^*)}{3(G(1,1) - G(0,1))},$ and let $\delta' := \delta(G(1,1) - G(0,1))$.
Note that $0 < \delta' < \frac{(G(1,1) - R^*)}{3}$.
Let $\alpha := \frac{c'}{(G(1,1) - R^* - 3\delta')} > 0$.
For any $t > t_1 := \max\{t_0, \alpha^{1/r} ,(\alpha \delta'/G(1,1))^{-1/r}\}$, let
$t^*(t) := t - \lfloor \alpha t^{r} \rfloor,$ 
where $\lfloor \cdot \rfloor$ is the floor function.
Note that since $t > \alpha^{1/r}$, we have $t^*(t) \geq 1$.
Let $\{\bm{J_s^*}\}$ be an i.i.d. sequence of Bernoulli($q^*$) random variables for $1 \leq s \leq t$.
Let $\bm{\widehat Q_s^*} := \frac{1}{s} \sum_{s' = 1}^s \bm{J_{s'}^*}$ denote the empirical average of this sequence at step $s$.
We state the following useful lemma.

\begin{lemma}
\label{lem: martingale_prop}
For the sequence $\{\bm{J_s^*}\}_{s \geq 1}$ defined above, and any $t \geq 1$, we have
    \begin{subequations}
    \begin{align}
        \mathbb{E}\left[\sum_{s = 1}^{t} G(f_s(\bm{(J^*)^{s-1}}), \bm{J_s^*}))\right] &= t R^* \text{ and } \label{eq:Gteq}\\
        \mathbb{E}\left[\sum_{s=1}^{t} \bm{J_s^*}\right] &= t q^* \label{eq:Jteq}.
    \end{align}
    \end{subequations}
\end{lemma}

See Appendix~\ref{sec: martingaleproof} for the proof of this lemma.
We define the sequence $\{\bm{J_s'}\}_{s=1}^{t}$ as specified in the statement of Proposition~\ref{prop:noregretsensitivity}.
In other words, we define $\bm{J_s'} = \bm{J^*_s}$ for $1 \leq s \leq t^*(t)$, and $\bm{J_s'} = 1$ for $t^*(t) < s \leq t$.
Then, we can denote the empirical average of this sequence as $\bm{\widehat Q_s'} := \frac{1}{s} \sum_{s' = 1}^s \bm{J_{s'}'}$ for $1 \leq s \leq t$.
We denote
\begin{align}
\label{eq: M_def}
M := \frac{1}{\lfloor \alpha t^{r} \rfloor} \cdot \mathbb{E}\left[\sum_{s = 1}^{\lfloor \alpha t^{r} \rfloor} G\left(f_{t^*(t) + s}\left(\bm{(J')^{t^*(t) + s - 1}}\right),1\right)\right].
\end{align}
From the definition of uniform no-regret, i.e. Equation~\eqref{eq: suff_large_no_regret}, we have
\begin{align*}
    c'
    &\geq \frac{1}{t^{r}} \cdot \mathbb{E} \l[T \max\{G(0,\bm{\widehat Q_t'}), G(1,\bm{\widehat Q_t'})\} - \sum_{s = 1}^{t} G(f_s(\bm{(J')^{s-1}}), \bm{J_s'})) \r] \\
    &\geq \frac{1}{t^{r}} \cdot \mathbb{E} \l[t \cdot G(1,\bm{\widehat Q_t'}) - \sum_{s = 1}^{t} G(f_s(\bm{(J')^{s-1}}), \bm{J_s'})) \r] \\
    &= \frac{1}{t^{r}} \cdot \l[ t^*(t) \cdot R^* + \lfloor \alpha t^{r} \rfloor \cdot G(1,1) - t^*(t) \cdot R^* - \lfloor \alpha t^{r} \rfloor \cdot M \r] \\
    &\geq (G(1,1) - M) \alpha -  G(1,1) t^{-r}.
\end{align*}
Using the fact that $\alpha := \frac{c'}{(G(1,1) - R^*_1 - 3\delta')}$ and $t > \left(\frac{\alpha \delta'}{G(1,1)}\right)^{-1/r}$, we get


\begin{align*}
    M \geq G(1,1) - \frac{c'}{\alpha} - \frac{G(1,1) \cdot t^{-r}}{\alpha}
    = R^* + 3\delta' - \frac{G(1,1) \cdot t^{-r}}{\alpha}
    \geq R^* + 2\delta' .
\end{align*}
%
Now, using linearity of expectation, and linearity of the payoff function $G(p,1)$ in the argument $p$, we get
\begin{align*}
    M &= G(\overline{f}, 1) \text{ where } \\
    \overline{f} &:= \frac{1}{\lfloor \alpha t^r \rfloor}  \sum_{s = 1}^{\lfloor \alpha t^r \rfloor} \mathbb{E}\left[f_{t^*(t) + s}\left(\bm{(J')^{t^*(t) + s - 1}}\right)\right] .
\end{align*}
%
Now, since $G(1,1) > G(0,1)$, we note that $G(p,1) = G(0,1) + (G(1,1) - G(0,1)) p$ is an increasing function in $p$ and so we get
\begin{align*}
\overline{f} \geq p^* + \frac{2\delta'}{G(1,1) - G(0,1)} = p^* + 2 \delta, 
\end{align*}
%
from the above inequality on $M$.
Thus, there exists $s(t)$ such that $1 \leq s(t) \leq \lfloor \alpha t^{r} \rfloor$ and 
\begin{align}\label{eq:sensitivitycondition2}
    \bbE \l[ f_{t^*(t) + s(t)}\left(\bm{(J')^{t^*(t) + s(t) - 1}}\right) \r] \geq p^* + 2\delta.
\end{align}
To write this in the language of Equation~\eqref{eq:sensitivitycondition}, we observe that
\begin{align*}
    0 < \frac{s(t)}{t^*(t) + s(t)} \leq \frac{\lfloor \alpha t^{r} \rfloor}{t^*(t) + \lfloor \alpha t^{r} \rfloor} \leq \frac{\alpha t^{r}}{t} = \alpha t^{r-1} \leq \alpha (t^*(t) + s(t))^{r-1}, 
\end{align*}
%
and therefore we get
\begin{align}\label{eq:stinequality}
    s(t) \leq \alpha (t^*(t) + s(t))^{r} .
\end{align}

We note that $t^*(t) \to \infty$ as $t \to \infty$, and hence we can define an infinite sequence of integer tuples $\{t_k, s_k\}_{k \geq 1}$ (where we have defined $t_k = t^*(t_1 + k) + s_k$ and $s_k = s(t_1 + k)$ as above) such that $0 < s_k \leq \alpha (t_k)^{r}$ and
\begin{align}
\label{eq: twisted_response_exp}
\mathbb{E}\left[f_{t_k}\left(\bm{(J'(k))^{t_k}}\right)\right] \geq p^* + 2\delta \text{ for all } k = 1,2, \ldots
\end{align}
%
This is precisely the statement in Equation~\eqref{eq:sensitivitycondition}, and completes the proof of Proposition~\ref{prop:noregretsensitivity}.
\Halmos
\endproof
% \end{proof}

\subsection{Last-iterate divergence when opponent is already at equilibrium}\label{sec:warmup}

Equation~\eqref{eq:sensitivitycondition} highlights a critical property of any self-agnostic uniformly no-regret algorithm with a regret rate of $(r,c)$: 
it needs to be sufficiently sensitive to small perturbations on the order of $t^r$ in the opponent's strategy.
We can concretize this property to show last-iterate divergence when both players use optimal no-regret strategies, i.e. $r = 1/2$ satisfying Assumptions~\ref{as:meanbased} and~\ref{as:monotonic}, i.e. the mean-based and monotonic assumptions.
Recall that under the mean-based assumption, player $1$'s strategy functions are given by

\begin{align}\label{eq:empiricalaverages}
f_t(\bm{(J)^{t-1}}) := f_t(\bm{\widehat{Q}_{t-1}}) \text{ for all } t \geq 1 .
\end{align}

The mean-based assumption underlies the broad family of Online-Mirror-Descent algorithms that satisfy the external-no-regret property.
More generally, strategies that use an appropriate mean of the past history of outcomes are among the earliest algorithms satisfying related properties\footnote{Note, however, that most algorithms that satisfy these latter properties are not self-agnostic, and so we do not study their properties here. } like Blackwell approachability~\citep{blackwell1956}, internal-no-regret~\citep{blum2007external} and calibration~\citep{foster1998asymptotic}.
Moreover, in reality, for our techniques to work we only need strategies to be mean-based in an approximate sense.
In other words, in Section~\ref{sec:optimism} we show that essentially the same results hold when the players use variants of the above class of strategies that incorporate a \textit{recency bias}.

The way we will show last-iterate-divergence for player $1$ is in the style of \textit{proof-by-contradiction}: we show that if player $2$ were able to converge in the last-iterate, player $1$ \textit{must} diverge.
The central idea is that the stochasticity in the realizations of player $2$, itself, cause player $1$ to diverge.
This result in its full generality is in Section~\ref{sec:lastiteratedivergence}.
Here, we state and prove a warm-up result that most clearly illustrates how the stochasticity in realizations \textit{alone} can lead to last-iterate divergence.
This considers the special case where player $2$ is playing his equilibrium strategy at all steps, i.e. $\{\bm J_t\}_{t \geq 1} \text{ i.i.d} \sim \text{Bernoulli}(q^*)$.
Remarkably, we show that even this simple case necessitates the limiting mixed strategy of player $1$ to diverge!
(This is in stark contrast to the setting of telepathic dynamics, in which a simple algorithm like multiplicative weights used in the matching pennies game would lead player $1$ to converge to the NE strategy, $p^* = 1/2$.)
\vidyacomment{For now I'm keeping all text here as-is, but we will return to discussing the discrepancy between a fixed strategy by player $2$ and an adaptive one in subsequent sections.}

\begin{theorem}\label{thm:warmup}
    Let player $2$'s strategy $\{\bm{J_t}\}_{t \geq 1}$ be an i.i.d. sequence of Bernoulli($q^*$) random variables.
    Then, any mean-based repeated game strategy $\{f_t\}_{t \geq 1}$ that has a regret rate of $(1/2,c)$ causes player $1$'s last iterate to diverge, i.e. there exist positive constants $(\delta,\epsilon)$ such that
    \begin{align}
    \label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon .
    \end{align}
\end{theorem}
% The proof of Theorem~\ref{thm:warmup} constitutes an elementary application of Markov's inequality, and a change-of-measure argument on the probability mass functions of two binomial random variables.
The proof of Theorem~\ref{thm:warmup} constitutes an elementary application of Markov's inequality and the central limit theorem, and is provided below.

\input{tex/proof_warmup}

\subsection{Main result: Last-iterate oscillations when \textit{both} players use no-regret}

The case for which player $2$ is \textit{already} at equilibrium serves to isolate the ramifications of the stochasticity in realizations.
While the day-to-day behavior of players is clearly quite different when both players are using popular no-regret strategies (see Figures~\ref{fig:MPoptimalfixedNE} and~\ref{fig:MPoptimalstochastic} in Section~\ref{sec:simulations} for a comparison), we show below that the inherent stochasticity in realizations continues to be the dominating factor in last-iterate oscillations.
\begin{theorem}\label{thm:lastiteratedivergence}
If both players $1$ and $2$ use mean-based and monotonic, optimal-no-regret repeated game strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$, respectively, then the pair of mixed strategies of both the players $(\bm{P_t}, \bm{Q_t})$ cannot converge almost surely.
\end{theorem}

\input{tex/proof_martingale}

\subsection{Extensions beyond the mean-based assumption}\label{sec:optimism}
\label{sec: beyond_mean_based}

\vidyacomment{To be edited}

In this section, we examine the fidelity of these last-iterate divergence results beyond exact mean-based strategies (Assumption~\ref{as:meanbased}).
While the mean-based assumption is fairly strong, it is worth noting that mean-based strategies underlie the design of almost all no-regret algorithms in practice.
Moreover, as we will now show, the essence of our results continues to hold even for algorithmic variants of mean-based strategies that are ubiquitous in the online learning and games literature.

One of the most common such variants incorporates a form of recency bias, colloquially called ``optimism''.
We define the broad class of recency-bias strategies below.
\begin{definition}\label{def:krecencybias}
The class of $\ell$-recency bias strategies is defined as below:
\begin{align*}
f_t(\bm{J^{t-1}}) := f_t(\bm{\widehat{Q}^\ell_{t-1}}) \text{ where } \\
\bm {\widehat{Q}^\ell_t} := \frac{1}{t} \left(\sum_{s=1}^{t} \bm{J_s} + \sum_{j = 1}^{\ell} r_j \bm{J_{t - j + 1}}\right) ,
\end{align*}
%
and $\{r_j\}_{j=1}^\ell$ are positive integers taking values in $\{1,\ldots, \ell\}$.
\end{definition}

Note that the class of $0$-recency bias strategies essentially constitutes mean-based strategies, and $1$-recency bias strategies with $r_1 = 1$ constitutes the class of \textit{optimistic} mean-based strategies, since they are using $\sum_{s=1}^t \bm{J_s} + \bm{J_t}$ as the summary statistic.

As mentioned in Section~\ref{sec: intro}, the study of the last iterate of optimism-based strategies has generated a lot of interest in the optimization literature~\citep{daskalakis2018training,mertikopoulos2018optimistic,liang2019interaction,abernethy2019last,lei2020last}; more-over, these strategies are known to cause faster time-averaged convergence~\citep{rakhlin2013optimization,syrgkanis2015fast}.
Most recently, it was shown that the last iterate of the players' strategies in the setting of telepathic dynamics (that arises when players use each others' mixtures to update their strategies) will converge~\citep{daskalakis2018last}.
In the more realistic realization model, the following result shows that the ensuing stochasticity \textit{alone} causes recency-bias-based strategies to diverge.

\begin{theorem}\label{thm:optimism}
 Assume that player $2$'s strategy $\{\bm{J_t}\}_{t \geq 1}$ is an i.i.d. sequence of Bernoulli($q^*$) random variables.
    Then, any $\ell$-recency-bias strategy $\{f_t\}_{t \geq 1}$, as defined in Definition~\ref{def:krecencybias}, that has a regret rate of $(1/2,c)$  causes player $1$'s last iterate to diverge, i.e. there exist positive constants $(\delta,\epsilon)$ such that
    \begin{align}
    \label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon .
    \end{align}
\end{theorem}


The proof of Theorem~\ref{thm:optimism} is essentially a relatively simple variant of the proof of Theorem~\ref{thm:warmup} with slightly more involved algebraic calculations of the involved probability mass functions owing to the recency bias.
The full proof is contained in Appendix~\ref{sec: optimismproof}.
It is worth noting that the bounded memory of the recency bias, as well as bounded increments $\{r_j\}_{j=1}^{\ell}$ are critical to the essence of the argument.
It is plausible that stronger recency biases that grow with the number of steps $t$ could lead to different last-iterate behavior; however, such stronger recency biases could also break the no-regret property.

\subsection{Open questions and conjectures}\label{sec:lastiteratedivergence}

\vidyacomment{To be edited}
Now, we ask what will happen if both the players use a mean-based optimal no-regret repeated game strategy, say given by the sequences of functions $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ respectively.
This generates a probability distribution on the set of sequences $\{I_t, J_t\}_{t \geq 1}$.

Suppose that we could show that the induced distribution on the empirical average of player $2$, i.e. $\bm{\widehat Q_t}$, was similar to a (normalized) Binomial random variable, i.e. $\bm{Z_t}/t$, in the following sense:
% Suppose the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are such that 
\begin{align}
\label{eq: req_measure_ratio_prop}
 \frac{\bbP(t\bm{\widehat Q_t} = z)}{\bbP(\bm{Z_t} = z)} \geq \epsilon_1 \text{  for all } z \in [tq^* - \beta' \sqrt{t}, tq^* + \beta \sqrt{t}],
\end{align}
for some $\epsilon_1 > 0$, for all $t$ sufficiently large (here, $\beta$ is as defined in the previous subsection).
Then, using the same ``change-of-measure'' argument as in the proof of Theorem~\ref{thm:warmup}, we would get
    $\bbP\left[\bm{P_{t_k}} \geq p^* + \delta \right] \geq (\epsilon_1 \epsilon)/2$, for all $k$ sufficiently large.
We conjecture that when the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are mean-based and satisfy optimal no-regret, the property~\eqref{eq: req_measure_ratio_prop} will hold.
This in turn would imply the following remarkable result.

\begin{conjecture}\label{con:lastiteratedivergence}
If both players $1$ and $2$ use self-agnostic, mean-based repeated game strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$, respectively, that are uniformly no-regret and each have a regret rate of $(1/2,c)$, 
then the pair of mixed strategies of both the players $(\bm{P_t}, \bm{Q_t})$ diverges with a positive probability.
\end{conjecture}

Observe that it is sufficient to show divergence of the pair $(\bm{P_t}, \bm{Q_t})$ from only the equilibrium $(p^*, q^*)$ with a positive probability.%
\footnote{This is because if a sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ did converge to some other point $(p, q) \neq (p^*, q^*)$, then the time-averages $(\bm{\hat P_t}, \bm{\hat Q_t})_{t \geq 1}$ would have to converge to $(p,q)$ as well.
However, we know that the time-averages have to converge to the equilibrium $(p^*, q^*)$ almost surely; thus the event that the sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ converges to some point other than the equilibrium has zero probability.}
% Hence to prove the conjecture, it is enough to prove that the sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ does not converge to the equilibrium with a positive probability.
In particular, it suffices to show that there exist positive constants $(\delta,\epsilon)$ such that
\begin{subequations}\label{eq:lastiteratedivergence}
    \begin{align}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] &\geq \epsilon     \text{ or } \label{eq:lastiteratedivergence1} \\
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{Q_{t}} - q^*| \geq \delta \right] &\geq \epsilon .\label{eq:lastiteratedivergence2}
    \end{align}
\end{subequations}



While we do not prove this conjecture, let us provide some intuition for it.
Suppose player $2$'s strategies results in him using a sequence of mixed strategies $\{\bm q_t\}_{t \geq 1}$ as an instance of randomness in the two players' strategies.
If this sequence does not converge, to $q^*$ then we cannot have last-iterate convergence and we are done.
The more interesting case is when the sequence $\{\bm q_t\}_{t \geq 1}$ converges to $q^*$.
Now, as a consequence of the optimal no-regret strategies of both the players, one can show that after sufficiently many steps the empirical average of player $2$'s action realizations is concentrated in an interval of length $\mathcal{O}(1/\sqrt{t})$ around $q^*$ at step $t$.
Also, player $2$ will be playing mixed actions $q_t$ close to $q^*$ for all $t$ sufficiently large.
In particular, his mixed actions will be bounded away from the pure actions, since his NE strategy $q^* \in (0,1)$.
As a result, it is unlikely that player $2$ would be able to have a precise control over the empirical average of his realized actions.
Thus, we would expect the condition in Equation~\eqref{eq: req_measure_ratio_prop},  which we call the \emph{shaky-hands} property, to hold.
This property is more formally defined below.

{\bf Shaky-hands property:}
    The mean-based strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are such that for any $\gamma > 0$, there exists an $\epsilon > 0$ and a $T > 0$ such that
\begin{align*}
 \frac{\bbP(t\bm{\hat Q_t} = z)}{\bbP(\bm{Z_t} = z)} \geq \epsilon \text{  for all } z \in [tq^* - \gamma \sqrt{t}, tq^* + \gamma \sqrt{t}],
\end{align*}
for all $t \geq T$.

The following proposition, whose proof is a straightforward consequence of the argument in the proof of Theorem~\ref{thm:warmup}, shows that strategies satisfying this shaky-hands property will automatically cause last-iterate divergence.

\begin{proposition}
    If the mean-based strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ satisfy the Shaky-hands property, and the strategy $\{f_t\}_{t \geq 1}$ of player $1$ has a regret-rate of $(1/2,c)$, then player $1$'s last-iterates diverge from the equilibrium strategy $p^*$, i.e. there exist positive constants $(\delta,\epsilon_0)$ such that
    \begin{align}
    %\label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon_0 .
    \end{align}
\end{proposition}
\begin{proof}

First, we carry over steps directly from the proof of Theorem~\ref{thm:warmup}.
We showed that
\[
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z_{t_k}} \leq q^* \cdot t_k + \beta \sqrt{t_k} \r) \geq \epsilon, 
\]
for all $k$ sufficiently large (here, $\epsilon$ is as defined in the previous subsection).
Let $\beta' > 0$ be such that 
\[
    \bbP \l({Z_t} < q^* t_k - {\beta'}{\sqrt{t}}\r) \leq \frac{\epsilon}{2},  
\]
for sufficiently large $t$.
Recall that $\bm Z_t \sim \text{Binomial}(t, q^*)$ and hence such $\beta'$ exists.
Then, we have
\begin{equation}
\label{eq: prob_f_Z_int}
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z_{t_k}} \in [q^* t_k - \beta' \sqrt{t_k}, q^* \cdot t_k + \beta \sqrt{t_k}] \r) \geq \frac{\epsilon}{2}, 
\end{equation}
for sufficiently large $k$, and where $\beta$ is defined as in the proof of Theorem~\ref{thm:warmup}.

Then, Equation \eqref{eq: req_measure_ratio_prop} follows from the shaky-hands property taking $\gamma = \max\{\beta', \beta\}$.
Taking $\epsilon_0 = \epsilon \epsilon_1/2$, we get the required result.
\end{proof}


\subsubsection{A comment on adaptive strategies}

Unfortunately, proving that player $2$'s iterates satisfy the shaky-hands property when both players using optimal-no-regret strategies is non-trivial.
The difficulty is primarily technical: the realizations of player $2$ are not mutually independent due to the adaptivity of player $2$.
However, the iterates $\{\bm{Q_t}\}_{t \geq 1}$ do \textit{marginally} satisfy certain favorable conditions that would result in the shaky-hands property if the realizations were independent.
To capture this, Theorem~\ref{thm:lastiteratedivergenceoblivious} in Appendix~\ref{sec:fixedconvergent} shows that the shaky-hands property holds for \textit{a-priori fixed} sequences $\{q_t\}_{t \geq 1}$ satisfying these conditions.
This implies last-iterate divergence of player $1$ when player $2$ plays non-adaptively.

More generally, nothing in our techniques precludes dependencies across realizations, as long as the probability mass function of player $2$'s sum of realizations at any step sufficiently resembles the probability mass function of a sum of mutually independent coin tosses.
Thus, we do believe that Theorem~\ref{thm:lastiteratedivergenceoblivious} implies last-iterate divergence for the full stochastic dynamical system.
However, the generality of our algorithmic framework, and minimal assumptions made on the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ will necessitate new mathematical techniques to formally prove this result.
%Add back \cb and \ck here in draft.
{Under an additional natural assumption on monotonicity on $\{f_t\}_{t \geq 1}$ (increasing in their arguments), we show in the sequel that the ``shaky hands" property is replaced by a condition on the cumulative distribution function of the empirical averages that is technically easier to reason about.
Then, we can show last-iterate divergence of the entire dynamical system.
Showing this last-iterate divergence in the absence of this monotonicity assumption, however, remains an intriguing open direction for future work.}


==> tex/result_noregret.tex.tex <==
%!TEX root = ../main.tex

\section{Main results}\label{sec:results}

In this section, we use the above assumptions to prove, in a series of steps, that the limiting mixed strategies as an outcome of both players using self-agnostic, mean-based, optimal no regret learning \textit{diverge}.
We start by proving a condition that any self-agnostic, optimal no-regret strategy necessarily satisfies (regardless of whether it is mean-based or not).
As described in Section~\ref{sec: intro}, this condition is described as sensitivity to \textit{fluctuations} in the time-average of the opponent strategy, and is detailed below.

\begin{figure}
    \centering
        \includegraphics[width=0.8\textwidth]{./Figures/sensitivity_figure_proof_2}
    \caption{Response of player $1$, who is using the multiplicative weights algorithm with learning rate $\eta = 1/\sqrt{t}$, against player $2$ who uses the randomized sequence in Equation~\eqref{eq:randomsequence}.
    The blue line plots the time-averages of player $2$, i.e. $\{\bm{\widehat Q_t}\}_{t \geq 1}$, and the red line plots the iterates of player $1$, i.e. $\{\bm P_t\}_{t \geq 1}$.
    Note that the $y$-axis of the figure is on linear scale, so the fluctuation in the time-averages of player $2$ is not visible.
    }\label{fig:sensitivity_figure_proof}
\end{figure}

\begin{proposition}\label{prop:noregretsensitivity}
For any self-agnostic repeated game strategy $\{f_t\}_{t \geq 1}$ used by player $1$ that is uniformly no-regret with a rate of $(r,c)$ 
(where $1/2 \leq r < 1$)
, and any $0 < \delta < (1 -p^*)/3$, there exists a positive constant $\alpha$ and an infinite sequence of integer tuples $\{(t_k,s_k)\}_{k \geq 1}$ such that
\begin{equation}
\label{eq:sensitivitymargin}
    0 < s_k \leq \alpha (t_k)^{r}, \text{ for all } k \geq 1,
\end{equation}
and
\begin{align}\label{eq:sensitivitycondition}
\mathbb{E}\left[f_{t_k}\left(\bm{(J'(k))^{t_k}}\right)\right] \geq p^* + 2\delta, \text{ for all } k \geq 1 ,
\end{align}
where the expectation is over the random sequence $\bm{(J'(k))^{t_k}} := \{\bm{J'_s(k)}\}_{s=1}^{t_k}$ defined as below:
\begin{align}\label{eq:randomsequence}
\bm{J'_s(k)} = \begin{cases}
\bm{J^*_s} \text{ i.i.d. } \sim \text{Bernoulli}(q^*), \text{ if } 1 \leq s \leq t_k - s_k, \\
1 \text{ otherwise. }
\end{cases}
\end{align}
\end{proposition}

In particular, if the self-agnostic repeated game strategy $\{f_t\}_{t \geq 1}$ is \textit{optimally} uniformly no-regret i.e. $r = 1/2$, then condition~\ref{eq:sensitivitymargin} would be
\[
   0 < s_k \leq \alpha \sqrt{t_k}, \text{ for all } k \geq 1. 
\]
For this case, Figure~\ref{fig:sensitivity_figure_proof} shows player $1$'s response, when she uses the multiplicative weight algorithm, to an opponent who plays the random sequence as defined in Equation~\eqref{eq:randomsequence}.
The game that is played is the matching pennies game, which is a zero-sum game with $G(0,0) = G(1,1) = 1$ and $G(0,1) = G(1,0) = 1$.
Her strategy, averaged over player $2$'s realizations, is shown to deviate sizably from the NE of the matching pennies game, $p^* = 0.5$.

This case is important because, even if player $2$ remained close to her equilibrium mixed strategy $q^*$ (as is \textit{necessary} in any hypothetical scenario of last-iterate convergence), there is a non-trivial probability of player $2$'s empirical average deviating from $q^*$ by a number on the order of $1/\sqrt{t}$ at step $t$.
The sensitivity in an optimal no-regret strategy to pick deviations of this order will allow us to show the non-convergence of player $1$'s mixed strategies in the subsequent Sections~\ref{sec:warmup},~\ref{sec:lastiteratedivergence} and~\ref{sec:optimism}.

\proof{Proof.}
Recall that by the competitive $2 \times 2$ game assumption, we have $G(0,1) < G(1,1)$.
Thus, for any $0 \leq p < 1$, we have $G(p,1) < G(1,1)$.
Consider $\{f_t\}_{t \geq 1}$ to be any self-agnostic uniformly no-regret strategy with a no-regret rate of $(r,c)$.
We note that for any $t$, and any sequence $\{J_s\}_{s=1}^t$, we have 
$$\max_{i \in \{0,1\}} \sum_{s=1}^t G(i,J_s) = t \cdot \max\{G(0,\widehat Q_t), G(1,\widehat Q_t)\}.$$
%
Thus, for $c' > c$, there exists a sufficiently large $t_0$ such that for all $t \geq t_0$, we have
\begin{equation}
\label{eq: suff_large_no_regret}
    \frac{1}{t^{r}} \l[t \cdot \max\{G(0,\widehat Q_t), G(1,\widehat Q_t)\} - \sum_{s = 1}^t G(f_s((J)^{s-1}), J_s)) \r] \leq c',
\end{equation}
for any sequence $\{J_s\}_{s = 1}^t$.

Recall that $R^*$ denotes the Nash equilibrium payoff of player $1$.
Because the equilibrium $(p^*,q^*)$ is strictly mixed, we have $R^* = G(p^*,q^*) = G(p^*, 1) < G(1,1)$.
Let $0 < \delta < \frac{(1 - p^*)}{3} = \frac{(G(1,1) - R^*)}{3(G(1,1) - G(0,1))},$ and let $\delta' := \delta(G(1,1) - G(0,1))$.
Note that $0 < \delta' < \frac{(G(1,1) - R^*)}{3}$.
Let $\alpha := \frac{c'}{(G(1,1) - R^* - 3\delta')} > 0$.
For any $t > t_1 := \max\{t_0, \alpha^{1/r} ,(\alpha \delta'/G(1,1))^{-1/r}\}$, let
$t^*(t) := t - \lfloor \alpha t^{r} \rfloor,$ 
where $\lfloor \cdot \rfloor$ is the floor function.
Note that since $t > \alpha^{1/r}$, we have $t^*(t) \geq 1$.
Let $\{\bm{J_s^*}\}$ be an i.i.d. sequence of Bernoulli($q^*$) random variables for $1 \leq s \leq t$.
Let $\bm{\widehat Q_s^*} := \frac{1}{s} \sum_{s' = 1}^s \bm{J_{s'}^*}$ denote the empirical average of this sequence at step $s$.
We state the following useful lemma.

\begin{lemma}
\label{lem: martingale_prop}
For the sequence $\{\bm{J_s^*}\}_{s \geq 1}$ defined above, and any $t \geq 1$, we have
    \begin{subequations}
    \begin{align}
        \mathbb{E}\left[\sum_{s = 1}^{t} G(f_s(\bm{(J^*)^{s-1}}), \bm{J_s^*}))\right] &= t R^* \text{ and } \label{eq:Gteq}\\
        \mathbb{E}\left[\sum_{s=1}^{t} \bm{J_s^*}\right] &= t q^* \label{eq:Jteq}.
    \end{align}
    \end{subequations}
\end{lemma}

See Appendix~\ref{sec: martingaleproof} for the proof of this lemma.
We define the sequence $\{\bm{J_s'}\}_{s=1}^{t}$ as specified in the statement of Proposition~\ref{prop:noregretsensitivity}.
In other words, we define $\bm{J_s'} = \bm{J^*_s}$ for $1 \leq s \leq t^*(t)$, and $\bm{J_s'} = 1$ for $t^*(t) < s \leq t$.
Then, we can denote the empirical average of this sequence as $\bm{\widehat Q_s'} := \frac{1}{s} \sum_{s' = 1}^s \bm{J_{s'}'}$ for $1 \leq s \leq t$.
We denote
\begin{align}
\label{eq: M_def}
M := \frac{1}{\lfloor \alpha t^{r} \rfloor} \cdot \mathbb{E}\left[\sum_{s = 1}^{\lfloor \alpha t^{r} \rfloor} G\left(f_{t^*(t) + s}\left(\bm{(J')^{t^*(t) + s - 1}}\right),1\right)\right].
\end{align}
From the definition of uniform no-regret, i.e. Equation~\eqref{eq: suff_large_no_regret}, we have
\begin{align*}
    c'
    &\geq \frac{1}{t^{r}} \cdot \mathbb{E} \l[T \max\{G(0,\bm{\widehat Q_t'}), G(1,\bm{\widehat Q_t'})\} - \sum_{s = 1}^{t} G(f_s(\bm{(J')^{s-1}}), \bm{J_s'})) \r] \\
    &\geq \frac{1}{t^{r}} \cdot \mathbb{E} \l[t \cdot G(1,\bm{\widehat Q_t'}) - \sum_{s = 1}^{t} G(f_s(\bm{(J')^{s-1}}), \bm{J_s'})) \r] \\
    &= \frac{1}{t^{r}} \cdot \l[ t^*(t) \cdot R^* + \lfloor \alpha t^{r} \rfloor \cdot G(1,1) - t^*(t) \cdot R^* - \lfloor \alpha t^{r} \rfloor \cdot M \r] \\
    &\geq (G(1,1) - M) \alpha -  G(1,1) t^{-r}.
\end{align*}
Using the fact that $\alpha := \frac{c'}{(G(1,1) - R^*_1 - 3\delta')}$ and $t > \left(\frac{\alpha \delta'}{G(1,1)}\right)^{-1/r}$, we get


\begin{align*}
    M \geq G(1,1) - \frac{c'}{\alpha} - \frac{G(1,1) \cdot t^{-r}}{\alpha}
    = R^* + 3\delta' - \frac{G(1,1) \cdot t^{-r}}{\alpha}
    \geq R^* + 2\delta' .
\end{align*}
%
Now, using linearity of expectation, and linearity of the payoff function $G(p,1)$ in the argument $p$, we get
\begin{align*}
    M &= G(\overline{f}, 1) \text{ where } \\
    \overline{f} &:= \frac{1}{\lfloor \alpha t^r \rfloor}  \sum_{s = 1}^{\lfloor \alpha t^r \rfloor} \mathbb{E}\left[f_{t^*(t) + s}\left(\bm{(J')^{t^*(t) + s - 1}}\right)\right] .
\end{align*}
%
Now, since $G(1,1) > G(0,1)$, we note that $G(p,1) = G(0,1) + (G(1,1) - G(0,1)) p$ is an increasing function in $p$ and so we get
\begin{align*}
\overline{f} \geq p^* + \frac{2\delta'}{G(1,1) - G(0,1)} = p^* + 2 \delta, 
\end{align*}
%
from the above inequality on $M$.
Thus, there exists $s(t)$ such that $1 \leq s(t) \leq \lfloor \alpha t^{r} \rfloor$ and 
\begin{align}\label{eq:sensitivitycondition2}
    \bbE \l[ f_{t^*(t) + s(t)}\left(\bm{(J')^{t^*(t) + s(t) - 1}}\right) \r] \geq p^* + 2\delta.
\end{align}
To write this in the language of Equation~\eqref{eq:sensitivitycondition}, we observe that
\begin{align*}
    0 < \frac{s(t)}{t^*(t) + s(t)} \leq \frac{\lfloor \alpha t^{r} \rfloor}{t^*(t) + \lfloor \alpha t^{r} \rfloor} \leq \frac{\alpha t^{r}}{t} = \alpha t^{r-1} \leq \alpha (t^*(t) + s(t))^{r-1}, 
\end{align*}
%
and therefore we get
\begin{align}\label{eq:stinequality}
    s(t) \leq \alpha (t^*(t) + s(t))^{r} .
\end{align}

We note that $t^*(t) \to \infty$ as $t \to \infty$, and hence we can define an infinite sequence of integer tuples $\{t_k, s_k\}_{k \geq 1}$ (where we have defined $t_k = t^*(t_1 + k) + s_k$ and $s_k = s(t_1 + k)$ as above) such that $0 < s_k \leq \alpha (t_k)^{r}$ and
\begin{align}
\label{eq: twisted_response_exp}
\mathbb{E}\left[f_{t_k}\left(\bm{(J'(k))^{t_k}}\right)\right] \geq p^* + 2\delta \text{ for all } k = 1,2, \ldots
\end{align}
%
This is precisely the statement in Equation~\eqref{eq:sensitivitycondition}, and completes the proof of Proposition~\ref{prop:noregretsensitivity}.
\Halmos
\endproof
% \end{proof}

\subsection{Last-iterate divergence when opponent is already at equilibrium}\label{sec:warmup}

Equation~\eqref{eq:sensitivitycondition} highlights a critical property of any self-agnostic uniformly no-regret algorithm with a regret rate of $(r,c)$: 
it needs to be sufficiently sensitive to small perturbations on the order of $t^r$ in the opponent's strategy.
We can concretize this property to show last-iterate divergence when both players use optimal no-regret strategies, i.e. $r = 1/2$ satisfying Asssumptions~\ref{as:meanbased} and~\ref{as:monotonic}, i.e. the mean-based and monotonic assumptions.
Recall that under the mean-based assumption, player $1$'s strategy functions are given by

\begin{align}\label{eq:empiricalaverages}
f_t(\bm{(J)^{t-1}}) := f_t(\bm{\widehat{Q}_{t-1}}) \text{ for all } t \geq 1 .
\end{align}

The mean-based assumption underlies the broad family of Online-Mirror-Descent algorithms that satisfy the external-no-regret property.
More generally, strategies that use an appropriate mean of the past history of outcomes are among the earliest algorithms satisfying related properties\footnote{Note, however, that most algorithms that satisfy these latter properties are not self-agnostic, and so we do not study their properties here. } like Blackwell approachability~\citep{blackwell1956}, internal-no-regret~\citep{blum2007external} and calibration~\citep{foster1998asymptotic}.
Moreover, in reality, for our techniques to work we only need strategies to be mean-based in an approximate sense.
In other words, in Section~\ref{sec:optimism} we show that essentially the same results hold when the players use variants of the above class of strategies that incorporate a \textit{recency bias}.

The way we will show last-iterate-divergence for player $1$ is in the style of \textit{proof-by-contradiction}: we show that if player $2$ were able to converge in the last-iterate, player $1$ \textit{must} diverge.
The central idea is that the stochasticity in the realizations of player $2$, itself, cause player $1$ to diverge.
This result in its full generality is in Section~\ref{sec:lastiteratedivergence}.
Here, we state and prove a warm-up result that most clearly illustrates how the stochasticity in realizations \textit{alone} can lead to last-iterate divergence.
This considers the special case where player $2$ is playing his equilibrium strategy at all steps, i.e. $\{\bm J_t\}_{t \geq 1} \text{ i.i.d} \sim \text{Bernoulli}(q^*)$.
Remarkably, we show that even this simple case necessitates the limiting mixed strategy of player $1$ to diverge!
(This is in stark contrast to the setting of telepathic dynamics, in which a simple algorithm like multiplicative weights used in the matching pennies game would lead player $1$ to converge to the NE strategy, $p^* = 1/2$.)
\vidyacomment{For now I'm keeping all text here as-is, but we will return to discussing the discrepancy between a fixed strategy by player $2$ and an adaptive one in subsequent sections.}

\begin{theorem}\label{thm:warmup}
    Let player $2$'s strategy $\{\bm{J_t}\}_{t \geq 1}$ be an i.i.d. sequence of Bernoulli($q^*$) random variables.
    Then, any mean-based repeated game strategy $\{f_t\}_{t \geq 1}$ that has a regret rate of $(1/2,c)$ causes player $1$'s last iterate to diverge, i.e. there exist positive constants $(\delta,\epsilon)$ such that
    \begin{align}
    \label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon .
    \end{align}
\end{theorem}
% The proof of Theorem~\ref{thm:warmup} constitutes an elementary application of Markov's inequality, and a change-of-measure argument on the probability mass functions of two binomial random variables.
The proof of Theorem~\ref{thm:warmup} constitutes an elementary application of Markov's inequality and the central limit theorem, and is provided below.

\input{tex/proof_warmup}

\subsection{Main result: Last-iterate oscillations when \textit{both} players use no-regret}

The case for which player $2$ is \textit{already} at equilibrium serves to isolate the ramifications of the stochasticity in realizations.
While the day-to-day behavior of players is clearly quite different when both players are using popular no-regret strategies (see Figures~\ref{fig:MPoptimalfixedNE} and~\ref{fig:MPoptimalstochastic} in Section~\ref{sec:simulations} for a comparison), we show below that the inherent stochasticity in realizations continues to be the dominating factor in last-iterate oscillations.
\begin{theorem}\label{thm:lastiteratedivergence}
If both players $1$ and $2$ use mean-based and monotonic, optimal-no-regret repeated game strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$, respectively, then the pair of mixed strategies of both the players $(\bm{P_t}, \bm{Q_t})$ cannot converge almost surely.
\end{theorem}

\input{tex/proof_martingale}

\subsection{Extensions beyond the mean-based assumption}\label{sec:optimism}
\label{sec: beyond_mean_based}

\vidyacomment{To be edited}

In this section, we examine the fidelity of these last-iterate divergence results beyond exact mean-based strategies (Assumption~\ref{as:meanbased}).
While the mean-based assumption is fairly strong, it is worth noting that mean-based strategies underlie the design of almost all no-regret algorithms in practice.
Moreover, as we will now show, the essence of our results continues to hold even for algorithmic variants of mean-based strategies that are ubiquitous in the online learning and games literature.

One of the most common such variants incorporates a form of recency bias, colloquially called ``optimism''.
We define the broad class of recency-bias strategies below.
\begin{definition}\label{def:krecencybias}
The class of $\ell$-recency bias strategies is defined as below:
\begin{align*}
f_t(\bm{J^{t-1}}) := f_t(\bm{\widehat{Q}^\ell_{t-1}}) \text{ where } \\
\bm {\widehat{Q}^\ell_t} := \frac{1}{t} \left(\sum_{s=1}^{t} \bm{J_s} + \sum_{j = 1}^{\ell} r_j \bm{J_{t - j + 1}}\right) ,
\end{align*}
%
and $\{r_j\}_{j=1}^\ell$ are positive integers taking values in $\{1,\ldots, \ell\}$.
\end{definition}

Note that the class of $0$-recency bias strategies essentially constitutes mean-based strategies, and $1$-recency bias strategies with $r_1 = 1$ constitutes the class of \textit{optimistic} mean-based strategies, since they are using $\sum_{s=1}^t \bm{J_s} + \bm{J_t}$ as the summary statistic.

As mentioned in Section~\ref{sec: intro}, the study of the last iterate of optimism-based strategies has generated a lot of interest in the optimization literature~\citep{daskalakis2018training,mertikopoulos2018optimistic,liang2019interaction,abernethy2019last,lei2020last}; more-over, these strategies are known to cause faster time-averaged convergence~\citep{rakhlin2013optimization,syrgkanis2015fast}.
Most recently, it was shown that the last iterate of the players' strategies in the setting of telepathic dynamics (that arises when players use each others' mixtures to update their strategies) will converge~\citep{daskalakis2018last}.
In the more realistic realization model, the following result shows that the ensuing stochasticity \textit{alone} causes recency-bias-based strategies to diverge.

\begin{theorem}\label{thm:optimism}
 Assume that player $2$'s strategy $\{\bm{J_t}\}_{t \geq 1}$ is an i.i.d. sequence of Bernoulli($q^*$) random variables.
    Then, any $\ell$-recency-bias strategy $\{f_t\}_{t \geq 1}$, as defined in Definition~\ref{def:krecencybias}, that has a regret rate of $(1/2,c)$  causes player $1$'s last iterate to diverge, i.e. there exist positive constants $(\delta,\epsilon)$ such that
    \begin{align}
    \label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon .
    \end{align}
\end{theorem}


The proof of Theorem~\ref{thm:optimism} is essentially a relatively simple variant of the proof of Theorem~\ref{thm:warmup} with slightly more involved algebraic calculations of the involved probability mass functions owing to the recency bias.
The full proof is contained in Appendix~\ref{sec: optimismproof}.
It is worth noting that the bounded memory of the recency bias, as well as bounded increments $\{r_j\}_{j=1}^{\ell}$ are critical to the essence of the argument.
It is plausible that stronger recency biases that grow with the number of steps $t$ could lead to different last-iterate behavior; however, such stronger recency biases could also break the no-regret property.

\subsection{Open questions and conjectures}\label{sec:lastiteratedivergence}

\vidyacomment{To be edited}
Now, we ask what will happen if both the players use a mean-based optimal no-regret repeated game strategy, say given by the sequences of functions $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ respectively.
This generates a probability distribution on the set of sequences $\{I_t, J_t\}_{t \geq 1}$.

Suppose that we could show that the induced distribution on the empirical average of player $2$, i.e. $\bm{\widehat Q_t}$, was similar to a (normalized) Binomial random variable, i.e. $\bm{Z_t}/t$, in the following sense:
% Suppose the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are such that 
\begin{align}
\label{eq: req_measure_ratio_prop}
 \frac{\bbP(t\bm{\widehat Q_t} = z)}{\bbP(\bm{Z_t} = z)} \geq \epsilon_1 \text{  for all } z \in [tq^* - \beta' \sqrt{t}, tq^* + \beta \sqrt{t}],
\end{align}
for some $\epsilon_1 > 0$, for all $t$ sufficiently large (here, $\beta$ is as defined in the previous subsection).
Then, using the same ``change-of-measure'' argument as in the proof of Theorem~\ref{thm:warmup}, we would get
    $\bbP\left[\bm{P_{t_k}} \geq p^* + \delta \right] \geq (\epsilon_1 \epsilon)/2$, for all $k$ sufficiently large.
We conjecture that when the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are mean-based and satisfy optimal no-regret, the property~\eqref{eq: req_measure_ratio_prop} will hold.
This in turn would imply the following remarkable result.

\begin{conjecture}\label{con:lastiteratedivergence}
If both players $1$ and $2$ use self-agnostic, mean-based repeated game strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$, respectively, that are uniformly no-regret and each have a regret rate of $(1/2,c)$, 
then the pair of mixed strategies of both the players $(\bm{P_t}, \bm{Q_t})$ diverges with a positive probability.
\end{conjecture}

Observe that it is sufficient to show divergence of the pair $(\bm{P_t}, \bm{Q_t})$ from only the equilibrium $(p^*, q^*)$ with a positive probability.%
\footnote{This is because if a sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ did converge to some other point $(p, q) \neq (p^*, q^*)$, then the time-averages $(\bm{\hat P_t}, \bm{\hat Q_t})_{t \geq 1}$ would have to converge to $(p,q)$ as well.
However, we know that the time-averages have to converge to the equilibrium $(p^*, q^*)$ almost surely; thus the event that the sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ converges to some point other than the equilibrium has zero probability.}
% Hence to prove the conjecture, it is enough to prove that the sequence $(\bm{P_t}, \bm{Q_t})_{t \geq 1}$ does not converge to the equilibrium with a positive probability.
In particular, it suffices to show that there exist positive constants $(\delta,\epsilon)$ such that
\begin{subequations}\label{eq:lastiteratedivergence}
    \begin{align}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] &\geq \epsilon     \text{ or } \label{eq:lastiteratedivergence1} \\
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{Q_{t}} - q^*| \geq \delta \right] &\geq \epsilon .\label{eq:lastiteratedivergence2}
    \end{align}
\end{subequations}



While we do not prove this conjecture, let us provide some intuition for it.
Suppose player $2$'s strategies results in him using a sequence of mixed strategies $\{\bm q_t\}_{t \geq 1}$ as an instance of randomness in the two players' strategies.
If this sequence does not converge, to $q^*$ then we cannot have last-iterate convergence and we are done.
The more interesting case is when the sequence $\{\bm q_t\}_{t \geq 1}$ converges to $q^*$.
Now, as a consequence of the optimal no-regret strategies of both the players, one can show that after sufficiently many steps the empirical average of player $2$'s action realizations is concentrated in an interval of length $\mathcal{O}(1/\sqrt{t})$ around $q^*$ at step $t$.
Also, player $2$ will be playing mixed actions $q_t$ close to $q^*$ for all $t$ sufficiently large.
In particular, his mixed actions will be bounded away from the pure actions, since his NE strategy $q^* \in (0,1)$.
As a result, it is unlikely that player $2$ would be able to have a precise control over the empirical average of his realized actions.
Thus, we would expect the condition in Equation~\eqref{eq: req_measure_ratio_prop},  which we call the \emph{shaky-hands} property, to hold.
This property is more formally defined below.

{\bf Shaky-hands property:}
    The mean-based strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ are such that for any $\gamma > 0$, there exists an $\epsilon > 0$ and a $T > 0$ such that
\begin{align*}
 \frac{\bbP(t\bm{\hat Q_t} = z)}{\bbP(\bm{Z_t} = z)} \geq \epsilon \text{  for all } z \in [tq^* - \gamma \sqrt{t}, tq^* + \gamma \sqrt{t}],
\end{align*}
for all $t \geq T$.

The following proposition, whose proof is a straightforward consequence of the argument in the proof of Theorem~\ref{thm:warmup}, shows that strategies satisfying this shaky-hands property will automatically cause last-iterate divergence.

\begin{proposition}
    If the mean-based strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ satisfy the Shaky-hands property, and the strategy $\{f_t\}_{t \geq 1}$ of player $1$ has a regret-rate of $(1/2,c)$, then player $1$'s last-iterates diverge from the equilibrium strategy $p^*$, i.e. there exist positive constants $(\delta,\epsilon_0)$ such that
    \begin{align}
    %\label{eq: liminf_prob_dev_response}
        {\lim \sup}_{t \to \infty} \bbP\left[|\bm{P_{t}} - p^*| \geq \delta \right] \geq \epsilon_0 .
    \end{align}
\end{proposition}
\begin{proof}

First, we carry over steps directly from the proof of Theorem~\ref{thm:warmup}.
We showed that
\[
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z_{t_k}} \leq q^* \cdot t_k + \beta \sqrt{t_k} \r) \geq \epsilon, 
\]
for all $k$ sufficiently large (here, $\epsilon$ is as defined in the previous subsection).
Let $\beta' > 0$ be such that 
\[
    \bbP \l({Z_t} < q^* t_k - {\beta'}{\sqrt{t}}\r) \leq \frac{\epsilon}{2},  
\]
for sufficiently large $t$.
Recall that $\bm Z_t \sim \text{Binomial}(t, q^*)$ and hence such $\beta'$ exists.
Then, we have
\begin{equation}
\label{eq: prob_f_Z_int}
    \bbP \l(f_{t_k} \l(\frac{\bm{{Z}_{t_k}}}{t_k} \r) \geq p^* + \delta, \bm{Z_{t_k}} \in [q^* t_k - \beta' \sqrt{t_k}, q^* \cdot t_k + \beta \sqrt{t_k}] \r) \geq \frac{\epsilon}{2}, 
\end{equation}
for sufficiently large $k$, and where $\beta$ is defined as in the proof of Theorem~\ref{thm:warmup}.

Then, Equation \eqref{eq: req_measure_ratio_prop} follows from the shaky-hands property taking $\gamma = \max\{\beta', \beta\}$.
Taking $\epsilon_0 = \epsilon \epsilon_1/2$, we get the required result.
\end{proof}


\subsubsection{A comment on adaptive strategies}

Unfortunately, proving that player $2$'s iterates satisfy the shaky-hands property when both players using optimal-no-regret strategies is non-trivial.
The difficulty is primarily technical: the realizations of player $2$ are not mutually independent due to the adaptivity of player $2$.
However, the iterates $\{\bm{Q_t}\}_{t \geq 1}$ do \textit{marginally} satisfy certain favorable conditions that would result in the shaky-hands property if the realizations were independent.
To capture this, Theorem~\ref{thm:lastiteratedivergenceoblivious} in Appendix~\ref{sec:fixedconvergent} shows that the shaky-hands property holds for \textit{a-priori fixed} sequences $\{q_t\}_{t \geq 1}$ satisfying these conditions.
This implies last-iterate divergence of player $1$ when player $2$ plays non-adaptively.

More generally, nothing in our techniques precludes dependencies across realizations, as long as the probability mass function of player $2$'s sum of realizations at any step sufficiently resembles the probability mass function of a sum of mutually independent coin tosses.
Thus, we do believe that Theorem~\ref{thm:lastiteratedivergenceoblivious} implies last-iterate divergence for the full stochastic dynamical system.
However, the generality of our algorithmic framework, and minimal assumptions made on the strategies $\{f_t\}_{t \geq 1}$ and $\{g_t\}_{t \geq 1}$ will necessitate new mathematical techniques to formally prove this result.
%Add back \cb and \ck here in draft.
{Under an additional natural assumption on monotonicity on $\{f_t\}_{t \geq 1}$ (increasing in their arguments), we show in the sequel that the ``shaky hands" property is replaced by a condition on the cumulative distribution function of the empirical averages that is technically easier to reason about.
Then, we can show last-iterate divergence of the entire dynamical system.
Showing this last-iterate divergence in the absence of this monotonicity assumption, however, remains an intriguing open direction for future work.}

